Beyond the Alphabet: Deep Signal Embedding for Enhanced DNA Clustering

The emerging field of DNA storage employs strands of DNA bases (A/T/C/G) as a storage medium for digital information to enable massive density and durability. The DNA storage pipeline includes: (1) encoding the raw data into sequences of DNA bases; (2) synthesizing the sequences as DNA \textit{strands} that are stored over time as an unordered set; (3) sequencing the DNA strands to generate DNA \textit{reads}; and (4) deducing the original data. The DNA synthesis and sequencing stages each generate several independent error-prone duplicates of each strand which are then utilized in the final stage to reconstruct the best estimate for the original strand. Specifically, the reads are first \textit{clustered} into groups likely originating from the same strand (based on their similarity to each other), and then each group approximates the strand that led to the reads of that group. This work improves the DNA clustering stage by embedding it as part of the DNA sequencing. Traditional DNA storage solutions begin after the DNA sequencing process generates discrete DNA reads (A/T/C/G), yet we identify that there is untapped potential in using the raw signals generated by the Nanopore DNA sequencing machine before they are discretized into bases, a process known as \textit{basecalling}, which is done using a deep neural network. We propose a deep neural network that clusters these signals directly, demonstrating superior accuracy, and reduced computation times compared to current approaches that cluster after basecalling.

==> newsections/0-abstract-barak.tex <==
The exponential growth of digital data has fueled interest in DNA as a storage medium due to its unmatched density and durability. However, clustering the billions of reads required for error correction and data reconstruction remains a major bottleneck, as traditional edit-distance-based methods are both computationally expensive and prone to data loss. This paper introduces a novel \emph{signal-model} that processes raw Nanopore signals, bypassing the error-prone basecalling step. By directly leveraging analog signal information, the \emph{signal-model} reduces computation time by up to three orders of magnitude compared to edit-distance approaches, while delivering superior accuracy. It also outperforms DNA sequence embedding methods in both accuracy and efficiency. Furthermore, our experiments show that the \emph{signal-model} achieves higher clustering accuracy than existing strand-based algorithms, saving days of computation without compromising quality. Overall, this work represents a significant breakthrough in DNA data storage, highlighting how signal-based analysis can drastically improve both accuracy and scalability.

==> newsections/1-introduction-barak-hadas.tex <==
Current storage technologies, such as magnetic disks and solid-state drives, are nearing their physical and scalability limits~\cite{carmean2018dna}, prompting the exploration of alternative solutions~\cite{chandak2020overcoming,rydning2022worldwide}. DNA has emerged as a promising alternative storage medium due to its exceptional density—~\cite{bornholt2016dna,erlich2017dna,goldman2013towards,yazdi2017portable} capable of storing exabytes of data per gram—and remarkable durability, enabling data preservation for thousands of years under optimal conditions.
\begin{figure}[t]
    \centering 
    \includegraphics[width=1\columnwidth]{figs/dna-storage-update11111.pdf}
    % \includegraphics[width=\linewidth]{figs/dna0-storage.pdf}
    \caption{Comparison of traditional DNA clustering pipelines and the proposed approach. The traditional method involves Nanopore sequencing followed by basecalling to generate discrete DNA reads. In contrast, our approach bypasses the basecalling step by directly clustering raw Nanopore signals, reducing errors and computational time.}   
    \label{fig:model}
\end{figure}
A DNA storage pipeline typically comprises four stages:
(i) \emph{encoding}, where binary data files are encoded into DNA strands (design files) using error-correcting codes (ECC)~\cite{koblitz2000state};
(ii) \emph{synthesis}, which produces artificial DNA strands for each design strand, subsequently stored in a \textit{storage container}~\cite{leproust2010synthesis};
(iii) \emph{sequencing}, where the stored DNA strands are translated back into noisy sequences known as \textit{``reads''}~\cite{anavy2019data,erlich2017dna,organick2018random,yazdi2017portable}; and
(iv) \emph{retrieval}, where clustering and reconstruction algorithms process the reads, decoding them back into binary data files while correcting errors using the selected coding methods. Among these stages, retrieval is particularly challenging due to the vast data scale and the sequencing errors introduced by current technologies.

Nanopore sequencing, the primary DNA sequencer used for DNA storage, enables real-time sequencing of DNA strands. The process involves a single DNA strand passing through a nanopore, causing variations in the measured ionic current. At any given time, the current primarily depends on a nucleotide subsequence of length 4–6 (i.e., a 6-mer) inside the pore. This raw current signal is sampled, resulting in a signal characteristic of the sequence~\cite{mao2018models,10409278}.

The signals are then processed by a \textit{basecaller}, which employs deep neural networks to translate the raw signals into nucleotide sequences composed of the bases {A, T, C, G}~\cite{10409278}. This translation is performed based on the most likely base sequence that could have induced the observed raw signals.

While Nanopore sequencing offers significantly lower costs and enhanced portability compared to traditional Illumina sequencing~\cite{jain2016oxford,kono2019nanopore}, it also presents several challenges: (1) higher sequencing error rates—approximately $10\%$ of bases suffer from edit, insertion, or deletion errors, compared to only $1\%$ in Illumina~\cite{chandak2020overcoming}; and (2) errors during the signal-to-read translation by the basecaller, which can exclude valid reads, reducing both accuracy and efficiency in downstream clustering and reconstruction tasks. Moreover, the sequencing and basecalling processes can take more than a week in some cases.

Clustering in this context has been explored solely for discrete DNA reads and involves clustering billions of strings\footnote{The number of clusters in DNA data storage typically ranges between $1,000$ and $100,000$, with each cluster containing between $10$ and $1,000$ samples.}. Most DNA clustering algorithms rely on the \textbf{edit distance} metric to identify groups of reads likely duplicated from the same source DNA strand. The edit distance between two strings \( x \) and \( y \), denoted as \( d_e(x, y) \), is defined as the minimum number of edits, deletions, or insertions required to transform \( x \) into \( y \)~\cite{ristad1998learning}. The core challenge of clustering DNA strands in DNA storage lies in the computation of a distance matrix based on the edit distance~\cite{landau1989fast}. This computation has a prohibitive quadratic complexity with respect to both the number and length of the reads, making it unscalable for typical DNA storage datasets, which are extremely large.

Our work addresses challenges in both Nanopore sequencing and clustering for DNA storage by proposing a paradigm shift: directly leveraging raw DNA signals for clustering, thereby bypassing the error-prone basecalling step (see Figure~\ref{fig:model}). Instead of searching for similarity in discrete DNA reads, our approach operates directly on raw analog DNA signals, which inherently contain richer contextual information. This enables more accurate clustering while minimizing information loss. Specifically, we replace computationally expensive edit-distance calculations with a deep neural network that learns an effective representation of DNA signals by embedding them into a similarity-preserving space. This significantly enhances both scalability and accuracy. We conduct extensive experiments on specialized datasets to demonstrate the effectiveness of our solution and its superior performance compared to DNA strand edit distance.

The key contributions of this work are as follows:
\begin{itemize}
\item We introduce a novel framework for directly clustering raw DNA signals during the retrieval stage, eliminating the need for extensive basecalling.
\item We develop a deep neural network that generates robust signal embeddings, ensuring high intra-cluster compactness and inter-cluster separability. This approach reduces sample exclusion and minimizes information loss.
\item We validate our approach on diverse datasets, achieving up to three orders of magnitude faster computation times compared to traditional methods, while maintaining clustering quality for accurate data reconstruction.
\end{itemize}

The remainder of this paper is organized as follows. 
Section~\ref{relatedwork} reviews related work. Section~\ref{method} details the proposed methodology, including both data processing and model design. Next, Section~\ref{eval} discusses our experimental setup and presents a thorough evaluation of results. Finally, Section~\ref{conclusion} concludes the paper.

==> newsections/2-related-work-barak-hadas.tex <==
Direct utilization of raw signals in DNA storage is challenging. To the best of our knowledge, no existing DNA storage approach directly exploits raw signal data for clustering, reconstruction, or error correction during the retrieval stage. Most prior clustering algorithms operate in the discrete domain and commonly employ edit-distance to compare DNA reads. This introduces high computational overhead rising from two factors: 
(i) \(\mathcal{O}(n^2)\) pairwise comparisons for \(n\) reads, and 
(ii) \(\mathcal{O}(\ell^2)\) per-comparison complexity, where \(\ell\) is the read length. 
Standard dynamic programming implementations of edit-distance~\cite{gusfield1997algorithms,landau1989fast} are prohibitively expensive at large scales, prompting various mitigation strategies. First, some methods limit the edit-distance depth~\cite{bao2011seed}. Second, others rely on fixed-sized short sub-strings (e.g., Starcode~\cite{zorita2015starcode}), and still others adopt heuristic-based similarity instead of exact edit-distance (e.g., Clover~\cite{qu2022clover}).

DNA clustering algorithms such as UCLUST~\cite{leproust2010synthesis}, CD-HIT~\cite{fu2012cd}, and USEARCH~\cite{srinivasavaradhan2021trellis} combine filtering and approximation strategies to reduce both the number of comparisons and the cost of each comparison. Filtering techniques include hashing approaches like Location Sensitive Hashing (LSH)~\cite{antkowiak2020low,ben2023gradhc,rashtchian2017clustering}, which group similar strands before performing explicit edit-distance computations. Although these clustering algorithms alleviate some computational bottlenecks, they still face scalability and accuracy trade-offs.


Moving to the signal domain, Dynamic Time Warping (DTW)~\cite{senin2008dynamic} is the time-series analogue of edit-distance, allowing insertions, deletions, and substitutions for sequences of different lengths. While DTW improves alignment flexibility, its base-case complexity is also quadratic. Despite further optimizations (e.g., limiting the warping window~\cite{rakthanmanon2012searching}), DTW remains impractical for many-to-many signal comparisons at a typical DNA storage datasets scale. Given that signals can be an order of magnitude longer than discrete DNA strands, DTW-based clustering suffers severely in performance.

A parallel line of work on DNA strand embeddings~\cite{fishman2023gena,ji2021dnabert,li2021bioseq} focuses on learning representations aligned with biological structures (e.g., proteins or genes). However, these embedding methods are task-specific and do not directly apply to synthetic DNA data storage, where the central goal is to recover the original data rather than to capture biological structures.

% DNA Storage Retrieval
% Discuss prior work on DNA storage, specifically in the context of the retrieval stage. Include methods that rely on clustering discrete DNA reads using edit-distance-based metrics and highlight their computational inefficiencies.

% Clustering Challenges expand on the computational and practical limitations of traditional clustering methods. Explain how existing approaches reduce complexity using filtering or approximation methods but often compromise on accuracy.

% Embedding-Based Approaches - Review literature on embedding-based methods for DNA sequence analysis, including those used in bioinformatics or metagenomics. Discuss their limitations in the context of synthetic DNA storage, where biological correctness (aligning to proteins) is not required.

% Signal Domain Analysis - Reference methods used for signal processing, such as Dynamic Time Warping (DTW), and explain why they are computationally impractical for large-scale DNA storage datasets. Highlight the lack of prior work that directly exploits raw DNA signals for clustering.

% Novelty of This Work Conclude by positioning your work as addressing the gaps in prior methods. Our approach is the first to cluster raw DNA signals directly



==> newsections/3-methodology-barak-hadas.tex <==
This section outlines the proposed framework for clustering raw DNA signals, focusing on the dataset creation, model architecture, and the integration of the ArcFace loss function to ensure robust and scalable embeddings.
\begin{table}[t!]
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Exp.} & \textbf{No.} & \textbf{Strand} & \textbf{Avg} & \textbf{Avg Strand} & \textbf{Creation} \\
& \textbf{Clusters} & \textbf{Length} & \textbf{Cluster} & \textbf{Length post} & \textbf{Time} \\
& & & \textbf{Size} & \textbf{Basecalling} & \textbf{[days]} \\
\midrule
Microsoft Exp. & 10,000 & 110 & 300 & 211 & 18 \\
Deep DNA Test & 110,000 & 140 & 10 & 243 & 30 \\
Deep DNA Pilot & 1,000 & 140 & 1,300 & 240 & 6 \\
\bottomrule
\end{tabular}}
\caption{Overview of experimental datasets and their key characteristics. The table shows the number of clusters, original strand length (in nucleotides), average cluster size (number of sequences per cluster), average strand length after basecalling, and dataset creation time in days.}
\label{tab:exptable}
\end{table}
\subsubsection{Dataset Construction}\label{sec:datacreate}
Public DNA storage datasets do not include raw signals, necessitating the creation of custom datasets that map raw signals to their corresponding DNA reads. To achieve this, experiments encompassing the four stages described in Section~\ref{intro} were conducted. These stages include \textit{encoding}, where error-correcting codes were applied to generate design files; \textit{synthesis}, using Twist Bioscience to produce DNA strands; \textit{sequencing}, performed with a Nanopore sequencer over approximately 72 hours; and \textit{basecalling}, translating raw signals into DNA reads, taking about one week. The final step involved creating the signal-strand datasets by calculating the edit distance between each DNA read and the original design strands.

Table~\ref{tab:exptable} summarizes three experiments used to construct these datasets~\footnote{The \say{Microsoft Experiment} design file is taken from~\cite{srinivasavaradhan2021trellis} and the sequenced data is from~\cite{sabary2024reconstruction}. The \say{Deep DNA Test} and \say{Deep DNA Pilot} design file and sequenced data are from ~\cite{bar2021deep}.}. The experiments varied in parameters such as the number of clusters, strand lengths, cluster size, and the coding scheme used to create the design files, ensuring diversity and robustness for evaluation. Each dataset's creation included a brute-force mapping of DNA reads to their original strands from the respective design file using edit-distance, which took between $6$ and $30$ days depending on the sequencing output size. These datasets provide a foundation for evaluating the model's ability to handle varying levels of complexity and sequencing errors.

\subsubsection{Architecture}
We propose a deep-learning-based algorithm to compute similarity between raw DNA signals, leveraging the pre-trained layers and weights of the Dorado basecaller~\cite{dorado2024}. Dorado is an open-source basecaller designed to translate raw electrical signals from Nanopore sequencing into nucleotide sequences. It employs a Conditional Random Field (CRF) architecture that includes convolutional, Long Short-Term Memory (LSTM)~\cite{yu2019review}, and linear layers. The convolutional layers extract salient features, the LSTM layers capture sequential dependencies, and the linear layers align the processed features to the output space. A Clamp layer ensures numerical stability by constraining prediction scores.

To adapt Dorado for clustering tasks, we truncate its architecture after the CRF layer, producing a $1024$-dimensional embedding vector. A linear layer with dimensions \(1024 \times 500\) is appended to map the embeddings to $500$ clusters, corresponding to the number of distinct clusters in the training set. This architecture is trained with the ArcFace loss (see Section~\ref{sec:loss} Loss Function), which enhances the discriminative power of the embeddings by enforcing compact intra-cluster structures and distinct inter-cluster separations.

The model processes raw DNA signals directly as input. Our architecture leverages Dorado's pre-trained feature extraction capabilities while incorporating clustering-specific components, enabling effective handling of noise and signal variability inherent in DNA data. This design produces robust embeddings suitable for large-scale clustering tasks.

\noindent \textbf{Training Framework.}
During training, we employed a fine-tuning approach by initializing our model weights with pre-trained weights of the Dorado model and then iteratively updating them during training using the Adam optimizer~\cite{kingma2014adam}. The model is trained on the \say{Microsoft Experiment} dataset, which contains $205,690$ samples from $500$ selected clusters. The data is split into \(70\%\) for training, \(15\%\) for validation, and \(15\%\) for testing. The performance is measured with a batch size of \(256\) on a AMD EPYC7513 server with 1TB RAM and four NVIDIA A6000 GPUs.

\subsubsection{Loss Function}\label{sec:loss}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{figs/softmaxarchface.png}
    \caption{Comparison between Norm-Softmax and ArcFace embeddings. Norm-Softmax projects feature vectors onto a hypersphere but does not enforce explicit angular separation, leading to smaller margins between classes. ArcFace introduces an angular margin, increasing inter-class separability and ensuring compact intra-class clustering~\citep{deng2019arcface}.}
    \label{fig:softarch}
\end{figure}

Traditional loss functions often struggle with embedding quality in noisy, high-dimensional DNA sequencing datasets. To address this, we implement ArcFace (Additive Angular Margin Loss)~\cite{deng2019arcface}, which optimizes embedding geometry on a hypersphere by introducing angular margin penalties between same-class embeddings~\cite{deng2019arcface,khan2024improvised}.

Let $\mathbf{x}_i \in \mathbb{R}^d$ be the deep feature of the $i$-th signal sample and $\mathbf{W}_j \in \mathbb{R}^d$ be the $j$-th column of weight matrix $\mathbf{W} \in \mathbb{R}^{d \times n}$, where embedding dimension $d=1024$ and number of classes $n=500$. The cosine similarity between $\mathbf{x}_i$ and $\mathbf{W}_j$ is: 
% \begin{equation}
$\cos(\theta_j) = \frac{\mathbf{W}_j^T \mathbf{x}_i}{\|\mathbf{W}_j\| \|\mathbf{x}_i\|}$.
% \end{equation}
The ArcFace loss function\footnote{$\cos(\theta_{y_i} + m) = \cos(\theta_{y_i})\cos(m) - \sin(\theta_{y_i})\sin(m)$} adds margin $m$ to the ground-truth class angle:
\begin{equation}
    L = -\frac{1}{N}\sum_{i=1}^N \log{\frac{e^{s\cos(\theta_{y_i} + m)}}{e^{s\cos(\theta_{y_i} + m)} + \sum_{j=1, j \neq y_i}^n e^{s\cos(\theta_j)}}}
\end{equation}
where $N$ is batch size and $s$ controls hypersphere radius. This normalization to a hypersphere with optimized angular distances ensures robust cluster separation, making it effective for DNA signal clustering. Figure~\ref{fig:softarch} demonstrates how ArcFace enforces compact intra-cluster embeddings while increasing angular separation between clusters.




% Traditional loss functions, such as cross-entropy and mean squared error, often fail to produce embeddings with high intra-cluster compactness and inter-cluster separability, particularly in noisy, high-dimensional datasets like those derived from DNA sequencing. To address these limitations, we employ ArcFace (Additive Angular Margin Loss)~\cite{deng2019arcface}, a state-of-the-art loss function designed to optimize embedding geometry on a hypersphere. Designed originally for face recognition tasks and is capable of handling tens of billions of classes (individual faces).

% ArcFace redefines similarity by introducing an angular margin penalty between embeddings of the same class, ensuring tighter intra-cluster distributions and wider inter-cluster separations~\cite{deng2019arcface,khan2024improvised}.  
% Let \(\mathbf{x}_i \in \mathbb{R}^d\) be the deep feature of the \(i\)-th signal sample, where $d=1024$ represents the embedding dimension before the final linear layer in a batch, belonging to the \(y_i\)-th class. Let \(\mathbf{W}_j \in \mathbb{R}^d\) denote the \(j\)-th column corresponding to class \(j\) of the weight matrix \(\mathbf{W} \in \mathbb{R}^{d \times n}\), where the embedding feature dimension \(d\) and the number of classes \(n\) are set to 1024 and 500, respectively, in this paper.  

% The cosine similarity between the feature vector \(\mathbf{x}_i\) of the \(i\)-th sample and the weight vector \(\mathbf{W}_j\) for class \(j\) is defined as:  $
%         \cos(\theta_j) = \frac{\mathbf{W}_j^T \mathbf{x}_i}{\|\mathbf{W}_j\| \|\mathbf{x}_i\|}
% $. ArcFace enhances class separability by modifying the similarity metric for the ground-truth class \(y_i\) through an additive angular margin \(m\). The ArcFace loss function\footnote{\(\cos(\theta_{y_i} + m) = \cos(\theta_{y_i})\cos(m) - \sin(\theta_{y_i})\sin(m)\).} is defined as:
% \begin{equation}
%     L = -\frac{1}{N}\sum_{i=1}^N \log{\frac{e^{s\cos(\theta_{y_i} + m)}}{e^{s\cos(\theta_{y_i} + m)} + \sum_{j=1, j \neq y_i}^n e^{s\cos(\theta_j)}}},
% \end{equation}
% where \(N\) denotes the batch size, \(s\) is a scaling factor that controls the hypersphere radius, and \(m\) represents the additive angular margin. This formulation normalizes feature embeddings to a hypersphere and optimizes angular distances between clusters, ensuring robust separability. The hyperparameters \(m\) and \(s\) were chosen from the original paper. Figure~\ref{fig:softarch} illustrates the benefits of ArcFace, showing how it enforces compact intra-cluster embeddings while increasing the angular separation between clusters. These properties make ArcFace particularly effective for DNA signal clustering, where precision and scalability are critical.


==> newsections/4-evaluation-barak-hadas.tex <==
\subsection{Experiments}
\hadas{a sentence defining the signal-model maybe earlier}
To evaluate the proposed approach, signal-model, we conducted experiments on subsets of $50$ clusters from each dataset: \emph{Deep DNA Pilot}, \emph{Deep DNA Test}, and \emph{Microsoft Experiment}. Each dataset contains both raw signals and the corresponding sequenced DNA reads, providing a comprehensive and diverse evaluation. These datasets vary significantly in size, with \emph{Deep DNA Pilot} subset containing $63,849$ samples, \emph{Deep DNA Test} subset containing $739$ samples, and \emph{Microsoft Experiment} subset containing $16,109$ samples. For each evaluation dataset, a binary ground truth matrix was constructed with its $50$ clusters, where the $[i,j]$ entry equals $1$ if and only if signals $i$ and $j$ belong to the same cluster.

% Notably, the \emph{Microsoft Experiment} subset clusters are different from the $500$ clusters used for training phase to serve as an unbiased evaluation set.

\subsection{Comparisons Results}\label{subsec:sompres}
In this section, we evaluate the performance of the signal-model's embedding-based similarity approach on DNA signals, comparing it to the edit-distance similarity method applied to DNA reads. The evaluation emphasizes both the accuracy of the similarity measure and the computational efficiency of the approaches.

To evaluate accuracy, we generated five distance matrices for each dataset. A cosine similarity matrix was created for the signal-model, as it is based on the ArcFace loss~\cite{deng2019arcface}. Additionally, four edit-distance matrices with varying depth constraints were generated. The depth constraint \(k\) determines the possible edit-distance values \(\{0, 1, \hdots, k\}\), where \(k\) sets the upper bound on insertions, deletions, or substitutions—higher values indicate greater dissimilarity.  

The chosen \(k\) values, \(10\), \(20\), \(50\), and \(200\), approximate \(5\%\), \(10\%\), \(25\%\), and \(100\%\) of the DNA read lengths, respectively. These constraints enable a fair comparison between the signal-model's embedding-based similarity and the edit-distance methods commonly used in DNA clustering algorithms. Non-heuristic-based algorithms, such as Starcode~\cite{zorita2015starcode}, Meshclust~\cite{james2018meshclust}, SEED~\cite{bao2011seed}, and Microsoft's alg~\cite{rashtchian2017clustering}, typically apply similar constraints or reduction techniques to balance computational efficiency and accuracy.  

Using these matrices, receiver operating characteristic (ROC) plots were generated. The ROC curve illustrates the trade-off between the true positive (TP) and false positive (FP) values of a ML model. Figure~\ref{fig:all_experiments} presents the ROC curves for the signal-model and the four baseline models with varying depth (\(k\)) values. Models with superior performance exhibit ROC curves closer to the top-left corner, indicating a higher TP rate and a lower FP rate. A random model aligns with the diagonal identity line, while the area under the ROC curve (AUC) quantifies performance, normalized to \([0,1]\), where \(1\) represents perfect classification.

The results demonstrate that the signal-model achieves higher \textbf{accuracy} than the strand-based models across all experiments. For the \say{Microsoft Experiment}, the signal-model attains an AUC of $0.99$, outperforming the strand-$k=200$ ($0.81$), strand-$k=50$ ($0.80$), strand-$k=20$ ($0.57$), and strand-$k=10$ ($0.51$).  

The sharp turn and linear increase in all curves reflect read pairs exceeding the $k$-threshold, rendering them equally distant. The strand-$k=200$ model is the closest in performance to the signal-model, as it effectively approximates an unbounded edit-distance calculation over the read length. However, this comes with significantly higher computational complexity.  

Similar trends appear for the \say{Deep DNA Pilot} and \say{Deep DNA Test} datasets (Figures~\ref{fig:all_experiments}(\subref{fig:omerrock}) and~\ref{fig:all_experiments}(\subref{fig:otherrock})). Notably, the \say{Microsoft Experiment} achieves superior performance because the evaluation clusters share the same data distribution as the training set, although the specific clusters used for evaluation were unseen during training.






\hadas{Lets talk about the threshold in comment- hadas footnote insert}
%For cosine similarity, the thresholds are continuous and not discrete as when using edit-distance, thus, containing much more data points, ranging between $-1$ and $1$, where $1$ is identical. 
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/mic_exp_roc_curve.pdf}
        \caption{\say{Microsoft Experiment}}
        \label{fig:microck}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/omer_exp_roc_curve.pdf}
        \caption{\say{Deep DNA Pilot}}
        \label{fig:omerrock}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/other_exp_roc_curve.pdf}
        \caption{\say{Deep DNA Test}}
        \label{fig:otherrock}
    \end{subfigure}
    \caption{Signal similarity vs. sequence similarity across the different experiments}
    \label{fig:all_experiments}
\end{figure*}

To compare computation times, Figure~\ref{fig:computation-time} illustrates the time required to compute similarity matrices for each model across all experiments. The differences between the signal-model and strand-models are shown on a logarithmic scale. For strand-$k=xx$ models, computation time corresponds to calculating the edit-distance similarity matrix, while for the signal-model, it includes the feed-forward process for generating embeddings and cosine similarity calculations. For the \say{Deep DNA Pilot} dataset, the computation time of the strand-$k=200$-model, marked with a cross, exceeds 30 hours. Notably, the strand-$k=xx$ models require \textbf{1 to 3 orders of magnitude} more time compared to the signal-model. Additionally, the strand-$k=xx$ models exhibit a linear increase in computation time as $k$ grows across all experiments. Variations in runtime across datasets are attributed to differences in dataset sizes processed by the same models.

\begin{figure}[!t]
        \includegraphics[width=1\linewidth, height=2in]{figforpaper/timing-dna111.pdf}
        \caption{Compute times for three different experiments. For the signal-model it includes both the embeddings and the cosine similarity computation times; for the different strand-$k=xx$-models it includes edit-distance similarity matrix computation time. The red cross indicates the omitted entries in which the running time is larger than 30 hours}
        \label{fig:computation-time}
\end{figure}

In summary, it appears that in terms of both accuracy and computation time, signal-model outperforms the strand-models.
\subsection{Compare to DNA embedding}
To further validate the significance of the paradigm shift from DNA reads to DNA signal we compare the proposed signal-model to three DNA strands embeddings models \textit{gena-lm-bert-base} , \textit{gena-lm-bert-large-t2t} from~\cite{fishman2023gena}, and \textit{DNABERT}~\cite{ji2021dnabert}. both \textit{DNABERT} and  \textit{gena-lm-bert-base} are $768$-dimensional embedding vector and \textit{gena-lm-bert-large-t2t} is $1024$-dimensional embedding like signal-model.
Figure~\ref{fig:all_experiments_rocLM} presents the ROC curves for the signal-model and the three DNA embedding models with the same baseline as in Section~\ref{subsec:sompres}. The comparisons clearly indicate that the representations obtained by our model are more distinguishable than the pre-trained DNA embedding models which demonstrate that the signal-model achieves higher \textbf{accuracy} than the strand-based embeddings across all experiments.
For the \say{Microsoft Experiment}, the signal-model attains an AUC of $0.99$, outperforming the \textit{gena-lm-bert-base} ($0.64$), \textit{gena-lm-bert-large-t2t} ($0.70$), strand-$k=20$ ($0.57$), and \textit{DNABERT} ($0.6$).Similar trends appear for the \say{Deep DNA Pilot} and \say{Deep DNA Test} datasets (Figures~\ref{fig:all_experiments_rocLM}(\subref{fig:omerrockLM}) and~\ref{fig:all_experiments_rocLM}(\subref{fig:otherrockLM})).

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figs/mic_exp_roc_curve_LM.pdf}
        \caption{\say{Microsoft Experiment}}
        \label{fig:microckLM}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figs/omer_exp_roc_curve_LM.pdf}
        \caption{\say{Deep DNA Pilot}}
        \label{fig:omerrockLM}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figs/other_exp_roc_curve_LM.pdf}
        \caption{\say{Deep DNA Test}}
        \label{fig:otherrockLM}
    \end{subfigure}
    \caption{Signal similarity vs. sequence Embedding similarity across the different experiments}
    \label{fig:all_experiments_rocLM}
\end{figure*}
\hadas{DO we need to explain more about those models?}
%GENA-LM is a Family of Open-Source Foundational Models for Long DNA Sequences. GENA-LM models are transformer masked language models trained on human DNA sequence.
%DNABERT: pre-trained Bidirectional Encoder Representations from Transformers model for DNA-language in genome

\subsection{Clustering Evaluation}
To demonstrate the potential of the signal-model's embeddings in traditional clustering algorithms, hierarchical clustering algorithm~\cite{murtagh2012algorithms}, which is compatible with cosine similarity, is applied. The performance of the clustering using the signal-model embeddings is summarized in Table~\ref{tab:clustertable}, which reports clustering metrics for the three datasets. The metrics include the Rand score, homogeneity, completeness, and the V-measure, providing a detailed analysis of the clustering quality. The Rand score evaluates the agreement between predicted and ground truth clusters by measuring the proportion of correctly grouped sample pairs. Across all datasets, the Rand score exceeds $88\%$, with near-perfect scores on the \emph{Microsoft Experiment} ($0.971$) and \emph{Deep DNA Test} ($0.978$). Homogeneity measures whether each cluster contains only samples of a single class, while completeness evaluates whether all samples of a class are assigned to the same cluster. Both metrics exhibit strong performance, particularly for the smaller datasets. The V-measure, a harmonic mean of homogeneity and completeness, demonstrates the overall clustering quality, with the \emph{Microsoft Experiment} achieving $0.866$ and the \emph{Deep DNA Test} achieving $0.839$. Although the \emph{Deep DNA Pilot} dataset shows slightly reduced performance, this is attributed to its larger size and increased complexity.

\begin{table}[t]
\centering
\footnotesize
\caption{Clustering scores for the three experiments using raw DNA signals.}
\label{tab:clustertable}
\begin{tabularx}{\columnwidth}{lYYYYY}
\toprule
\textbf{Dataset} & \textbf{Time [s]} & \textbf{Rand} & \textbf{Homogen.} & \textbf{Comp.} & \textbf{V-measure} \\
\midrule
Microsoft Experiment & 58      & 0.971 & 0.790 & 0.959 & 0.866 \\
Deep DNA Pilot       & 970.82  & 0.887 & 0.528 & 0.859 & 0.654 \\
Deep DNA Test        & 0.12    & 0.978 & 0.821 & 0.857 & 0.839 \\
\bottomrule
\end{tabularx}
\end{table}


Figure~\ref{fig:tsneall} provides tSNE visualizations of the signal-model across the three datasets, offering insights into the cluster separability achieved. In the \emph{Microsoft Experiment} (Figure~\ref{fig:tsneall}(\subref{fig:Tsnemic})), the clusters exhibit clear separations, benefiting from the consistency between the training and evaluation distributions. Conversely, the \emph{Deep DNA Pilot} dataset (Figure~\ref{fig:tsneall}(\subref{fig:Tsneomer})) shows denser and larger clusters due to its greater complexity and dataset size. The \emph{Deep DNA Test} dataset (Figure~\ref{fig:tsneall}(\subref{fig:Tsneother})) demonstrates sparse and smaller clusters, reflecting its simpler structure. These visualizations align with the quantitative metrics and validate the signal-model's capability to capture meaningful cluster structures.

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-mic50.pdf}
        \caption{\say{Microsoft Experiment}}
        \label{fig:Tsnemic}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-omer50.pdf}
        \caption{\say{Deep DNA Pilot}}
        \label{fig:Tsneomer}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-other50.pdf}
        \caption{\say{Deep DNA Test}}
        \label{fig:Tsneother}
    \end{subfigure}
    \caption{TSNE Analysis of 50 Clusters from Various Experiments}
    \label{fig:tsneall}
\end{figure*}


% The reconstruction phase further demonstrates the utility of the signal-model. Reconstruction relies on the output clusters, calculating error rates within each cluster and selectively removing reads to achieve a target error rate conducive to successful design file reconstruction~\cite{pan2022rewritable, sabary2024reconstruction}. Unlike traditional clustering methods, such as Clover~\cite{qu2022clover} and Microsoft's alg~\cite{rashtchian2017clustering}, which discard significant portions of the data, the signal-model retains all clusters while ensuring sufficient separability for downstream reconstruction. Clover, for instance, excludes $3\%$ of the samples and exhibits deviations in cluster sizes and counts, whereas Microsoft's method achieves higher accuracy but at the expense of significantly increased computation time and excluded reads. By retaining all data and producing well-separated clusters, the signal-model ensures that reconstruction algorithms are provided with a complete dataset, enabling efficient and accurate reconstruction.

% In summary, the signal-model achieves high clustering accuracy, as evidenced by both quantitative metrics and visualizations, while significantly reducing computational requirements. Unlike traditional approaches, it retains all clusters, thereby enhancing reconstruction capabilities and establishing itself as a robust and scalable solution for DNA storage pipelines.

\hadas{discuss the comparisons to other clustering algorithms in comment}
% Unlike modern DNA clustering algorithms which are commonly used, such as Clover~\cite{qu2022clover} and Microsoft's~\cite{rashtchian2017clustering}, the signal-model computation time is considerably faster. Additionally, we include all the raw signals samples, unlike for example Clover, which excludes $3\%$ of the strands samples. We compare the proposed signal-model to Clover, since Clover's execution time is the only one that is comparable in its execution time, however Clover's accuracy is significantly lower than the signal model's. The number of clusters that Clover returns is different from the actual number, $50$, and the number of samples in each cluster greatly differs from the ground truth. Microsoft's alg~\cite{rashtchian2017clustering} is orders of magnitude slower than Clover; see e.g.~\cite{ben2023gradhc,qu2022clover}, it also discards a notable number of reads, and similar to Clover, the number of clusters it produces does not align with the original cluster count, though its accuracy is higher. Both, Clover and Microsoft's alg, output a subset of highly distinguished clusters, while excluding many samples. Unlike them, Signal-model outputs clusters which are distinguishable enough so reconstruction can be done, across all clusters. 

==> newsections/4-new-evaluation.tex <==
We examine two aspects of the proposed signal-based approach. First, we analyze our signal embeddings through comparisons with both edit distance-based methods and existing DNA embedding models. Second, we assess the clustering performance of our approach through comprehensive representation and accuracy analyses. We conduct our evaluations on three diverse datasets: \emph{Microsoft Experiment}, \emph{Deep DNA Pilot}, and \emph{Deep DNA Test}.  The results demonstrate both the accuracy and computational advantages of our method compared to existing approaches.

\begin{table}[t!]
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset} & \textbf{Size} & \textbf{Cluster Size} & \textbf{Use Case} \\
\midrule
Microsoft Exp. & 16,109 & Medium  & Practical deployment \\
Deep DNA Test & 739 & Small  & Baseline performance \\
Deep DNA Pilot & 63,849 & Large  & Large-scale validation \\
\bottomrule
\end{tabular}
}
\caption{Overview of the three datasets created from the experiments.}
\label{TABLE_DATASETS}
\end{table}
From each dataset, we selected subsets containing $50$ clusters to ensure a balanced comparison while maintaining computational feasibility. As shown in Table~\ref{TABLE_DATASETS}, \emph{Deep DNA Pilot} ($63,849$ samples, large clusters) is our large-scale validation dataset and presents challenging conditions for data retrieval due to the huge cluster sizes. In contrast, \emph{Deep DNA Test} ($739$ samples, small clusters) provides a controlled baseline for evaluating performance presents challenges to learn embeddings that distinguish between clusters. Finally, \emph{Microsoft Experiment} ($16,109$ samples, medium clusters) strikes a balance in scale and practical deployment considerations. These distinct characteristics ensure a comprehensive assessment of DNA storage clustering methods.

Each dataset provides both DNA signals and their corresponding sequenced reads, enabling direct comparison. To evaluate, we constructed binary similarity matrices for each dataset, where matrix entry $[i,j]$ equals $1$ if signals $i$ and $j$ belong to the same cluster, and $0$ otherwise. This ground truth serves as the baseline for our quantitative analysis and allows for systematic evaluation of clustering accuracy.
\subsection{Performance Analysis of Signal Embeddings}
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/mic_exp_roc_curve.pdf}
        \caption{\say{Microsoft Experiment}}
        \label{fig:microck}
    \end{subfigure}
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/omer_exp_roc_curve.pdf}
        \caption{\say{Deep DNA Pilot}}
        \label{fig:omerrock}
    \end{subfigure}
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/other_exp_roc_curve.pdf}
        \caption{\say{Deep DNA Test}}
        \label{fig:otherrock}
    \end{subfigure}
    \caption{Comparison of DNA signal similarity with \textit{signal-model} embeddings and DNA sequence similarity with edit-distance across datasets.}
    \label{fig:all_experiments}
\end{figure*}
\subsubsection{Comparison with edit distance}
We evaluate the performance of the \textit{signal-model}'s embedding-based similarity approach against traditional edit-distance methods applied to DNA reads for clustering. The evaluation focuses on both accuracy and computational efficiency.

To assess accuracy, we generated five distance matrices for each dataset: one cosine similarity matrix for the \textit{signal-model} (based on ArcFace loss~\cite{deng2019arcface}) and four edit-distance matrices with varying depth constraints. The depth constraint $k$ determines the range of possible edit-distance values $\{0, 1, \ldots, k\}$, where $k$ bounds the number of allowed insertions, deletions, or substitutions. We selected $k$ values of $10$, $20$, $50$, and $200$, approximately corresponding to $5\%$, $10\%$, $25\%$, and $100\%$ of our experimental DNA storage reads length (see~Table \ref{tab:exptable}). 

\begin{figure}[!t]
    \centering
        \includegraphics[width=0.8\columnwidth]{figforpaper/timing-dna111.pdf}
        \caption{Computation times across three datasets. For the \textit{signal-model}, this includes embedding generation and cosine similarity calculations, while for strand-\(k=xx\) models it covers edit-distance computations. Red crosses mark entries where the runtime exceeded 30 hour.}
        \label{fig:computation-time}
\end{figure}

An important distinction between the methods lies in their similarity measures. While edit-distance provides discrete thresholds corresponding to specific numbers of edits, the \textit{signal-model}'s cosine similarity offers continuous values ranging from $-1$ to $1$, where $1$ indicates perfect similarity.

Using these matrices, receiver operating characteristic (ROC) plots were generated. The ROC curve illustrates the trade-off between the true positive (TP) and false positive (FP) values of an ML model. Figure~\ref{fig:all_experiments} presents ROC curves comparing the \textit{signal-model} against the four baseline models with varying depth ($k$) values. Models with better performance exhibit ROC curves closer to the top-left corner, indicating a higher TP rate and a lower FP rate. A random model aligns with the diagonal identity line, while the area under the ROC curve (AUC) quantifies performance, normalized to $[0,1]$, where $1$ represents perfect classification.

The results demonstrate that the \textit{signal-model} achieves higher accuracy than the strand-based models across all experiments. For the \say{Microsoft Experiment}, the \textit{signal-model} attains an AUC of $0.99$, significantly outperforming the strand-$k=200$ ($0.81$), strand-$k=50$ ($0.80$), strand-$k=20$ ($0.57$), and strand-$k=10$ ($0.51$) models. The sharp turn and linear increase in all curves reflect read pairs exceeding the $k$-threshold, rendering them equally distant. The strand-$k=200$ model is the closest in performance to the \textit{signal-model}, as it effectively approximates an unbounded edit-distance calculation over the read length. However, this comes with significantly higher computational complexity.

Similar trends appear for the \emph{Deep DNA Pilot} and \emph{Deep DNA Test} datasets (Figures~\ref{fig:all_experiments}(\subref{fig:omerrock}) and~\ref{fig:all_experiments}(\subref{fig:otherrock})). Notably, the \emph{Microsoft Experiment} achieves better performance because the evaluation clusters share the same data distribution as the training set, although the specific clusters used for evaluation were unseen during training.

Regarding computational efficiency, Figure~\ref{fig:computation-time} illustrates the time required for similarity matrix computation across all experiments. The \textit{signal-model} demonstrates remarkable efficiency, requiring \textbf{1 to 3 orders of magnitude less time} compared to strand-based approaches. For the strand-$k=xx$ models, computation times increase linearly with $k$, while the \textit{signal-model} maintains consistent performance regardless of sequence complexity.

\subsubsection{Comparison with DNA embedding models}
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/mic_exp_roc_curve_LM.pdf}
        \caption{\emph{Microsoft Experiment}}
        \label{fig:microckLM}
    \end{subfigure}
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/other_exp_roc_curve_LM.pdf}
        \caption{\emph{Deep DNA Test}}
        \label{fig:otherrockLM}
    \end{subfigure}
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/omer_exp_roc_curve_LM.pdf}
        \caption{\emph{Deep DNA Pilot}}
        \label{fig:omerrockLM}
    \end{subfigure}
    \caption{Comparison of DNA signal similarity with \textit{signal-model} embeddings and DNA sequence similarity using DNA embedding models across datasets.}
    \label{fig:all_experiments_rocLM}
\end{figure*}
To further validate the \textit{signal-model}'s approach, we compare against open sourced state-of-the-art DNA sequence embedding models: \textit{gena-lm-bert-base} (GLBB), \textit{gena-lm-bert-large-t2t} (GLBL)~\cite{fishman2023gena}, and \textit{DNABERT}~\cite{ji2021dnabert}. The GENA-LM models comprise a family of foundational models specifically designed for long DNA sequences, employing transformer-based architectures pre-trained on extensive human DNA sequence data. While the base version (GLBB) uses a standard BERT architecture, the large version (GLBL) incorporates additional transformer layers and attention mechanisms optimized for DNA sequences. DNABERT offers a specialized BERT model adapted for DNA sequences, incorporating $k$-mer embedding strategies to capture local sequence patterns. It employs a bidirectional encoder architecture specifically tuned for genomic data, with pre-training objectives designed to capture biological sequence properties.

In terms of embedding dimensionality, \textit{DNABERT} and \textit{gena-lm-bert-base} produce $768$-dimensional vectors, while \textit{gena-lm-bert-large-t2t} generates $1024$-dimensional embeddings matching our \textit{signal-model}'s dimensionality. While these models excel at capturing biologically relevant features in natural DNA sequences, they may not be optimally suited for synthetic DNA storage applications where the sequences don't necessarily follow natural biological patterns. 

Figure~\ref{fig:all_experiments_rocLM} presents ROC curves comparing these approaches, demonstrating the \textit{signal-model}'s superior performance across all experiments. For the \emph{Microsoft Experiment}, our model achieves an AUC of $0.99$, substantially outperforming GLBB ($0.64$), GLBL ($0.70$), and \textit{DNABERT} ($0.6$).

Table~\ref{DNA--TABLE} provides a unified comparison of both metrics, accuracy (AUC) and computational efficiency (Time), across four models on the three datasets. Our \textit{signal-model} approach significantly outperforms existing DNA models, achieving superior AUC scores ($0.92$--$0.99$) compared to ($0.6$--$0.7$) for the other DNA-based models. In terms of computational efficiency, our \textit{signal-model} processes the \emph{Microsoft Exp} dataset in $11.57$ seconds compared to $99$--$173$ seconds for other models, demonstrating up to 15x speedup while maintaining higher accuracy.
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Metric} & \textbf{GLBB} & \textbf{GLBL} & \textbf{DNABERT} & \textbf{\textit{signal-model}} \\
\midrule
\textbf{Microsoft Exp} & AUC & 0.64 & 0.70 & 0.60 & 0.99 \\
& Time[s] & 103.84 & 173.52 & 99.25 & 11.57 \\
\midrule
\textbf{Deep DNA Test} & AUC & 0.64 & 0.70 & 0.57 & 0.92 \\
& Time[s] & 1.56 & 3.53 & 3.00 & 1.49 \\
\midrule
\textbf{Deep DNA Pilot} & AUC & 0.60 & 0.70 & 0.56 & 0.94 \\
& Time[s] & 156.14 & 371.91 & 274.93 & 98.07 \\
\bottomrule
\end{tabular}}
\caption{Performance comparison of \textit{signal-model} and DNA embedding models across datasets.}
\label{DNA--TABLE}
\end{table}
\subsection{Clustering Performance Analysis}
To evaluate the \textit{signal-model}'s clustering capabilities, we conduct a systematic analysis across two key dimensions: representation quality and accuracy metrics. Our evaluation employs hierarchical clustering~\cite{murtagh2012algorithms} with cosine similarity on the three datasets, comparing against widely adopted DNA data storage clustering algorithms: Clover~\cite{qu2022clover} and Microsoft's alg~\cite{rashtchian2017clustering} (which we independently implemented following their paper's description), using their suggested parameters. Beyond demonstrating better clustering performance, our \textit{signal-model} approach eliminates the need for the time-consuming basecalling phase (saving days of computation), while achieving better results compared to DNA-based clustering algorithms. This shows that classical clustering techniques, when applied to our signal-based embeddings, can effectively outperform DNA storage clustering methods.

\subsubsection{Representation Learning}
Figure~\ref{fig:tsneall} provides t-SNE visualizations across the three datasets, offering insights into cluster separability. The \emph{Microsoft Experiment} (Figure~\ref{fig:tsneall}(a)) exhibits well-defined cluster boundaries with clear separation in the embedding space, demonstrating the model's ability to effectively distinguish between different clusters under typical conditions. The \emph{Deep DNA Test} results (Figure~\ref{fig:tsneall}(b)), despite its sparse data distribution, the visualization demonstrates clear cluster separation, with distinct groupings spread across the embedding space.Additionally, the \emph{Deep DNA Pilot} (Figure~\ref{fig:tsneall}(c)) shows denser cluster formations, reflecting the increased complexity and challenging conditions inherent in larger-scale data. These visualizations across different experimental conditions demonstrate the robustness of our \textit{signal-model}'s approach in capturing meaningful features within DNA signal data.
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.43\columnwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-mic50.pdf}
        \caption{\emph{Microsoft Experiment}}
        \label{fig:Tsnemic}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.43\columnwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-other50.pdf}
        \caption{\emph{Deep DNA Test}}
        \label{fig:Tsneother}
    \end{subfigure}
    \vspace{2mm}
    \begin{subfigure}[b]{0.43\columnwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-omer50.pdf}
        \caption{\emph{Deep DNA Pilot}}
        \label{fig:Tsneomer}
    \end{subfigure}
    \caption{t-SNE analysis of the 50 clusters of each dataset.}
    \label{fig:tsneall}
\end{figure}

\subsubsection{Clustering Accuracy for DNA} For evaluating clustering performance in DNA storage applications, traditional clustering metrics are insufficient as they do not account for the unique characteristics of DNA storage. We adopt and extend the accuracy measure introduced by~\cite{rashtchian2017clustering}, specifically designed for DNA storage data retrieval tasks. Let $C$ represent the ground truth clustering and $\tilde{C}$ denote the predicted clustering output from an algorithm. We define the clustering accuracy $\mathcal{A}_{\gamma,\beta}$ with two key parameters: $\gamma$ controlling the minimum required overlap for correct cluster identification, and $\beta$ establishing the maximum allowed fraction of false positives. Formally: \begin{definition}[DNA Storage Clustering Accuracy]
For clusters $C$, $\tilde{C}$, with parameters $0.5 < \gamma \leq 1$\text{,} $0\leq \beta < 0.5$\text{,} and a minimum overlap threshold $N$, the accuracy of $\tilde{C}$ with respect to $C$ is:
\begin{equation}
{\fontsize{9pt}{11pt}\selectfont
\begin{aligned}
    \mathcal{A}_{\gamma,\beta}(C, \tilde{C}) = \max_{\pi} \frac{1}{|C|} \sum_{i=1}^{|C|} &\mathbf{1}\{\tilde{C}_{\pi(i)} \setminus |\tilde{C}_{\pi(i)} \cap C_i| \leq \beta|\tilde{C}_{\pi(i)}| \\
    &\text{and } |\tilde{C}_{\pi(i)} \cap C_i| \geq \min(N, \gamma|C_i|)\}
\end{aligned}}
\end{equation}
where $\pi$ is a mapping from $\{1,2,\ldots,|C|\}$ to $\{1,2,\ldots,\max(|C|,|\tilde{C}|)\}$.
\end{definition}

This definition extends the original formulation in~\cite{rashtchian2017clustering} in two significant ways. First, we introduce the parameter $\beta$ to allow for a controlled fraction of false positives, considering that DNA storage reconstruction algorithms are designed to handle and correct a certain level of errors~\cite{sabary2024reconstruction}. Second, we add the constant $N$ to accommodate varying cluster sizes, particularly important for large-scale cluster size. ~\cite{rashtchian2017clustering}'s accuracy is defined for $\beta=0$ and under the assumption that the output of sequencing is a small number of noisy DNA reads of each cluster reference.

The accuracy measure $\mathcal{A}_{\gamma,\beta}$ evaluates clustering quality through two essential conditions. The false positive condition $\tilde{C}_{\pi(i)} \setminus |\tilde{C}_{\pi(i)} \cap C_i| \leq \beta|\tilde{C}_{\pi(i)}|$ ensures that no more than a $\beta$-fraction of elements in each predicted cluster are incorrectly assigned. Additionally, the overlap condition $|\tilde{C}_{\pi(i)} \cap C_i| \geq \min(N, \gamma|C_i|)$ requires either a minimum absolute overlap of $N$ samples or a relative overlap of $\gamma$-fraction, whichever is smaller. This interpretation justifies the need for high accuracy and an error fraction: each underlying cluster represents one stored unit of information.
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/mic_clustering_results.pdf}
        \caption{\emph{Microsoft Experiment}}
        \label{fig:micclust}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/other_clustering_results.pdf}
        \caption{\emph{Deep DNA Test}}
        \label{fig:otherclust}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/omer_clustering_results.pdf}
        \caption{\emph{Deep DNA Pilot}}
        \label{fig:omerclust}
    \end{subfigure}
    \caption{Comparison to Microsoft algorithm. Figures (a) and (b) plot $\mathcal{A}_{\gamma,\beta}$ for varying $\gamma \in \{0.6, 0.7, 0.8, 0.9, 1.0\}$ and $N=200$. (c) plots $\mathcal{A}_{\gamma,\beta}$ for varying $N\in\{20,50,100,200,400\}$ due to \emph{Deep DNA Pilot} huge clusters that in this case $N=\min(N, \gamma|C_i|)$. All figures include plots for $\beta\in \{0,0.1,0.2\}$ as the false positive rate in the clusters. In (a) and (c) our Alg $\beta=0.1$, our Alg $\beta=0.2$ have the same accuracy.}
    \label{fig:clustering_results}
\end{figure*}

Figure~\ref{fig:clustering_results} presents accuracy comparisons between our hierarchical clustering algorithm, which leverages signal-model embeddings, and Microsoft’s state-of-the-art method for DNA data storage sequences~\cite{rashtchian2017clustering}. Clover was excluded from this comparison because it consistently underperformed. Each subplot captures the performance under distinct datasets and parameter variations, illustrating how accuracy changes in response to the false-positive rate $\beta\in\{0,0.1,0.2\}$, the overlap determined by the min between the $\gamma$ threshold, and the constant parameter $N$. In particular, $\beta$ governs how much noise is introduced into each cluster (higher $\beta$ indicates noisier clusters), while $\gamma \in \{0.6, 0.7, 0.8, 0.9, 1.0\}$ in Figures~\ref{fig:clustering_results}~(a) and~\ref{fig:clustering_results}(b), specifying how strictly a produced cluster must overlap with the original ground-truth cluster. In Figure~\ref{fig:clustering_results}~(c), for the large cluster size dataset, we show accuracy as a function of \(N\), since the overlap is effectively determined by \(\min\bigl(N, \,\gamma \lvert C_i\rvert\bigr)\).

In Figure~\ref{fig:clustering_results}(a), our algorithm consistently achieves higher accuracy than Microsoft’s across all examined noise levels. While both methods experience slight decreases in accuracy under more stringent overlap requirements (larger $\gamma$), our algorithm remains comparatively robust, for smaller $\beta$ values our algorithm achieve $94\%$, while retaining accuracy above $60\%-70\%$ for larger $\beta$, whereas Microsoft’s method frequently hovers below $30\%$. In Figure~\ref{fig:clustering_results}(b), which corresponds to a smaller dataset, both algorithms show reduced performance due to tighter constraints on $\beta$ and $\gamma$. Nonetheless, our method still outperforms Microsoft’s: for $\beta=0.2$, we achieve $50\%$ accuracy versus Microsoft’s $30\%$. For both plots, $N$ is set to $200$, as it is enough for reconstruction purposes and does not affect the overlap fraction.

Finally, Figure~\ref{fig:clustering_results}(c) presents the results for the large dataset, where the effect of \(\gamma\) diminishes because \(N\) is effectively bounded by \(\min(N,\gamma|C_i|)\). Our algorithm achieves perfect accuracy at moderate \(N\) values and remains resilient even as \(N\) increases to 400. By contrast, Microsoft’s approach yields a vast majority of clusters of size~1 and merges many sequences into a few large clusters, resulting in stable but substantially lower accuracy overall. In fact, it creates 90\% of its clusters with size~1 and 97\% with sizes below~19, which are redundant given the dataset’s average cluster size of $1,300$. Moreover, in the few large clusters it does form, it often merges distinct groups, adversely affecting the \(\beta\) fraction and explaining the 20\% accuracy boost observed at \(\beta=0.2\). Nevertheless, that boost is overshadowed by the balanced cluster-size distribution our method maintains, as evidenced by its perfect accuracy for \(\beta=0.1\). Overall, these findings confirm that our hierarchical signal-model algorithm outperforms the existing state-of-the-art across various noise levels, overlap thresholds, and dataset sizes, underscoring its suitability for a successful reconstruction of DNA data storage tasks. 
\subsubsection{Clustering Robustness}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Dataset} & \textbf{Alg} & \textbf{Recall} & \textbf{Precision} & \textbf{F1} & \textbf{No. Clusters} \\
\midrule
\multirow{3}{*}{\textbf{Microsoft exp}} & \textit{signal-model} & 0.794 & 0.994 & 0.883 & 145 \\
& clover & 0.13 & 0.042 & 0.064 & 40 \\
& Mic. & 0.688 & 0.171 & 0.274 & 26 \\
\midrule
\multirow{3}{*}{\textbf{Deep DNA Test}} & \textit{signal-model} & 0.650 & 0.563 & 0.604 & 45 \\
& clover & 0.212 & 0.024 & 0.044 & 33 \\
& Mic. & 0.56 & 0.598 & 0.578 & 75 \\
\midrule
\multirow{3}{*}{\textbf{Deep DNA Pilot}} & \textit{signal-model} & 0.357 & 0.953 & 0.519 & 387 \\
& clover & 0.39 & 0.101 & 0.161 & 44 \\
& Mic. & 0.577 & 0.668 & 0.619 & 2090 \\
\bottomrule
\end{tabular}}
\caption{Comparison of clustering algorithms across datasets.}
\label{tab:clustering_comparison}
\end{table}
Table~\ref{tab:clustering_comparison} presents an evaluation of our algorithm against standard clustering metrics across all datasets. The performance is measured using three key metrics: Recall ($\frac{TP}{TP + FN}$), which indicates the model's ability to identify all positive samples; Precision ($\frac{TP}{TP + FP}$), which measures the model's accuracy in positive predictions; and F1 score, the harmonic mean of precision and recall that provides a balanced assessment of the model's overall performance.

The results demonstrate consistent strong performance across different experimental conditions. On the \emph{Microsoft Experiment} dataset, our algorithm achieves superior performance across all metrics. For the \emph{Deep DNA Test} dataset, while our and Microsoft algorithms show comparable performance, our approach maintains an edge in both Recall and F1 scores. Even on the challenging \emph{Deep DNA Pilot} dataset, which features exceptionally large clusters, our algorithm achieves a competitive F1 score of $0.519$ compared to Microsoft's $0.619$. Notably, while our and Microsoft algorithms process the complete dataset, Clover's approach discards a significant portion of the input reads—retaining only $3\%$ ($486$ of $16,109$) reads in the \emph{Microsoft Experiment} and less than $1\%$ ($476$ of $63,849$) in the \emph{Deep DNA Pilot}. We achieve similar results with Microsoft alg for Rand-Index ($0.98$), Homogeneity($\pm 0.8$), Completeness ($\pm 0.8$) and V-measure($\pm 0.8$) scores, while Clover does not.


==> newsections/5-conclusion-barak-hadas.tex <==
This work demonstrates the transformative potential of directly utilizing raw DNA signals in the analysis of Nanopore sequencing data, particularly for DNA storage applications. By leveraging a signal-based approach, our method achieves significant improvements in computational efficiency while maintaining high clustering accuracy. Our experimental results demonstrate the effectiveness of the signal-model's embeddings across multiple datasets, showing robust performance in generating discriminative representations that enable efficient clustering.

These findings underscore the importance of preserving raw signal information, often discarded during basecalling, for downstream DNA data storage tasks. Directly clustering raw signals may further reduce the risk of losing critical details essential for accurate data reconstruction. Future research could extend the signal-model to other sequencing applications—such as RNA—and investigate more advanced neural architectures for enhanced robustness. Moreover, specialized clustering algorithms and improved scalability techniques could unlock the full potential of this signal-based paradigm in DNA storage and beyond.

==> newsections/evaluation.tex <==
\subsection{Model Training}
During training, we employed a fine-tuning approach by initializing our model weights with pre-trained weights of the Dorado model and then iteratively updating them during training. For training purpose, $500$ clusters consisting of $205,690$ samples were selected arbitrarily from the \say{Microsoft Experiment} dataset whose size is in the magnitude of millions of samples. The samples are divided into three sets. The first contains $70\%$ of the samples, and it is used for training. The second contains $15\%$ of the samples, and it is used for validation, and the remaining $15\%$ are used for testing purposes, and to visualize the test set embedding. The ML models are trained with a batch size of 256 samples using the Adam optimizer~\citep{kingma2014adam}. During the first $50$ epochs of training, the training was conducted on a subset of 100 clusters, from the initial selected $500$. For the remaining $50$ epochs, training was conducted on all the clusters. When training on a large amount of data, using the ArcFace Loss, a common approach is to divide the training epochs, by gradually increasing the size of the training set ~\citep{khan2024improvised}. 

To evaluate the model, t-Distributed Stochastic Neighbor Embedding (tSNE) is used on the output's embeddings of the model, on the test set. tSNE is a dimensionality reduction technique utilized for visualizing high-dimensional data in lower-dimensional spaces, with an emphasis on preserving the local and global structure of the data points. Figure~\ref{fig:tsnetest} illustrates the visualization of tSNE on the test set, demonstrating a distinct separation between the different clusters.

The performance is measured on a 2x AMD EPYC 7513 (32 core) server with 1TB RAM and four NVIDIA A6000 GPUs.

\begin{figure}[ht]
        \centering
        \includegraphics[width=1\linewidth]{figforpaper/TSNE-testset.pdf}
        \caption{The test set is visualized using tSNE, with each color representing a distinct cluster. The presence of 500 clusters makes it difficult to distinguish similar colors visually. Each dot-like shape in the Figure represents a single cluster that is primarily well-separated from the other clusters.}
    \label{fig:tsnetest}
\end{figure}

\subsection{Experiments}
In this work, we perform experimental evaluations of our method on the three datasets we created, ensuring a comprehensive and diverse assessment as detailed in Section~\ref{sec:datacreate}. A subset of $50$ clusters was selected from each dataset. The \say{Deep DNA Pilot} dataset comprises $63,849$ samples, the \say{Deep DNA Test} dataset includes $739$ samples, and the \say{Microsoft Experiment} dataset contains $16,109$ samples, none of which were used during the training phase. To compare the experiments results a binary ground truth square matrix was constructed for each dataset. In this matrix, the $[i,j]$ entry equals $1$ only if the $i$ and $j$ signals belong to the same cluster.
\subsection{Comparisons Results}
In this section, we compare our model DNA signal similarity with DNA reads edit-distance similarity. 



Recall that when using edit-distance, the possible values are among $\{0, 1, \hdots, k\}$, where $k$ is the upper limit of insertion, deletion, or substitution. For each different $k$ value, an edit-distance similarity matrix is calculated, where a higher score entails a higher dissimilarity. The $k$ values chosen are $10$, $20$, $50$, and $200$; For example, for $k=10$, the tested thresholds set is $\{0,1,\ldots,10\}$, and for each threshold a prediction matrix is calculated. These values exemplify the typical approach taken by approximation-based DNA clustering algorithms to achieve faster computation times with minimal loss of accuracy. Such algorithms often use constraints or reduction techniques in edit-distance calculations (Starcode \citep{zorita2015starcode}, Meshclust \citep{james2018meshclust}, SEED \citep{bao2011seed} and Microsoft algorithm \citep{rashtchian2017clustering}). 

Every non-heuristic-based DNA clustering algorithm that measures similarity without direct computation relies on an edit-distance constraint. The ArcFace Loss ~\citep{deng2019arcface} uses a cosine similarity for separating between inputs, therefore, a cosine similarity matrix is created to compare every pair of signals. For cosine similarity, the thresholds are continuous and not discrete as when using edit-distance, thus, containing much more data points, ranging between $-1$ and $1$, where $1$ is identical. Using these matrices, receiver operating characteristic (ROC) is generated. The ROC curve illustrates the trade-off between the true positive (TP) and false positive (FP) values of a machine learning model.

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/mic_exp_roc_curve.pdf}
        \caption{\say{Microsoft Experiment}}
        \label{fig:microck}
    \end{subfigure}
    \begin{subfigure}[t]{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/omer_exp_roc_curve.pdf}
        \caption{\say{Deep DNA Pilot}}
        \label{fig:omerrock}
    \end{subfigure}
    \begin{subfigure}[t]{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/other_exp_roc_curve.pdf}
        \caption{\say{Deep DNA Test}}
        \label{fig:otherrock}
    \end{subfigure}
    \caption{Signal similarity vs. sequence similarity across the different experiments}
    \label{fig:all_experiments}
\end{figure*}

Figure~\ref{fig:all_experiments} shows the ROC curves for the proposed signal-model and the three different baselines that use edit-distance similarity of the DNA strands with varying values of $k$. We expect that models with better classification performance will have ROC curves closer to the top-left corner since this indicates high true positive rate with a small false positive. The curve of a random ML model is expected to be close to the diagonal identity line. We quantitatively measure this performance according to the area under the ROC curve (AUC) metric, normalized to $[0,1]$, where 1 indicates perfect classification.

Figure~\ref{fig:all_experiments} presents the ROC curve results for the three different experiments. The figure shows that the model that uses raw signals as inputs (signal-model) outperforms the models that use DNA strands as inputs (strand-$k=xx$) as higher TP rates are achieved for the same FP rates. Quantitatively, for the \say{Microsoft Experiment}, we find that the signal-model achieves the best trade-off between TP and FP with an AUC of $0.99$ as compared to $0.81$, $0.80$, $0.57$, and $0.51$ for the strand-$k=200$, the strand-$k=50$, the strand-$k=20$, and the strand-$k=10$ models, respectively. The sharp turn and linear increase across all the models, after the rapid rise, is attributed to read pairs with distance above $k$, thus, they are all treated as equally distant. The strand-$k=200$ is the only model that is comparable performance wise to the signal-model, though its complexity is much higher. Recall from Table \ref{fig:exptable}, the average strand's length is approximately $200$, therefore using an edit-distance with a $k=200$ value, can be treated as an unbounded edit-distance calculation. Similar trends can be seen for \say{Deep DNA Pilot} and \say{Deep DNA Test} (refer to Figures ~\ref{fig:all_experiments}(\subref{fig:omerrock}) and ~\ref{fig:all_experiments}(\subref{fig:otherrock}), respectively). Notice that the superior performance in the \say{Microsoft Experiment} compared to the other experiments is due to the training data originating from the same dataset. Even though the clusters that are used for evaluation were not present during the training process, the training process was conducted on the same dataset and thus the signals are taken from the same data distribution. 

\begin{figure}[!t]
        \includegraphics[width=1\linewidth, height=2in]{figforpaper/timing-dna111.pdf}
        \caption{Compute times for three different experiments. For the signal-model it includes both the embeddings and the cosine similarity computation times; for the different strand-$k=xx$-models it includes edit-distance similarity matrix computation time. The red cross indicates the omitted entries in which the running time is larger than 30 hours}
        \label{fig:computation-time}
\end{figure}

An important property of our similarity scheme is its execution time, as shown in Figure~\ref{fig:computation-time} on a logarithmic scale. It shows the computation time for the similarity matrices for each model, across all experiments. For the strand-$k=xx$ models, this entails the edit-distance similarity matrix computation time, and for the signal-model it entails the feed-forward that generates the embedding, and the cosine similarity calculation times. For the \say{Deep DNA Pilot} dataset, the computation time of the strand-$k=200$-model is marked using a red cross, because its computation time is larger than 30 hours. 

It is evident that the running time of strand-$k=xx$ models is between $1$ and $3$ orders of magnitude larger than that of signal-model. It is also evident that strand-$k=xx$ models have a linear increase between the different $k$ values across the different experiments. The variation between the datasets is due to the varying dataset sizes applied to the same model.

==> newsections/intro.tex <==
%what  is DNA STORAGE
The rapid growth of digital data, projected to reach $180$ zettabytes by 2025, is causing a data storage crisis that cannot be addressed by existing storage technologies~\citep{rydning2022worldwide,chandak2020overcoming}. In response, DNA is emerging as a promising alternative storage medium due to its incredible density and durability.
The DNA storage process includes four stages (1) an \textit{``encoding''} stage in which binary data files are encoded into DNA strands (design files) using error-correcting code (ECC) schemes that may also overcome errors~\citep{koblitz2000state}, (2) a \textit{``synthesis''} stage, which produces artificial DNA strands of each design strand and are then stored in a \textit{storage container}~\citep{leproust2010synthesis}, (3) a \textit{``sequencing''} stage~\citep{anavy2019data, erlich2017dna, organick2018random, yazdi2017portable} which translates a DNA strand into a sequence known as a \textit{``read''}, and (4) a \textit{“retrieval”} stage where clustering and reconstruction algorithms process the reads, the output is decoded back into binary data files while correcting errors using the selected coding methods.


%NANOPORE
%the challenges error rate and time of basecalling

The primary DNA sequencer used for DNA storage is Nanopore, which enables real-time sequencing of DNA strands. The sequencing process involves a single strand of DNA passing through a pore leading to variations in a measured ionic current. The current at any given time primarily depends on a nucleotide subsequence of length 4-6 (i.e., a 6-mer) inside
the pore at that instant. This raw current signal is sampled leading to generating a signal characteristic of the sequence ~\citep{mao2018models,10409278}. The signals are then processed by a \textit{basecaller}, which uses deep neural networks to translate them into nucleotide sequences composed of the bases ${A, T, C, G}$ ~\citep{10409278} based on the most likely base sequence that could have induced the raw signal. While offering significantly lower costs and enhanced portability compared to traditional Illumina sequencing~\citep{jain2016oxford, kono2019nanopore} it also poses several challenges due to the higher sequencing error rates (approximately $10\%$ of bases suffer from edit, insertion or deletion errors as compared to only $1\%$ in Illumina)~\citep{chandak2020overcoming}. Moreover, The sequencing and basecalling processes take more than a week in some cases.



%Clustering in DNA
%introduce the 4 challenges

A major stage in the DNA storage pipeline is clustering which has been explored solely in the context of clustering the discrete DNA reads and involves clustering billions\footnote{The clusters number in DNA data storage is typically between $1,000$ and $100,000$, while each cluster contains between $10$ and $1,000$ samples.} of strings based on the edit distance metric to identify which groups of reads were likely duplicated from the same source DNA strand. The edit distance between two strings $x$,$y$ denoted as $d_e(x,y)$ is the minimum number of edits, deletions, or insertions required to transform $x$ to $y$~\citep{ristad1998learning}.
The complexity of this procedure is caused by several factors: (1) The variability and probabilistic nature of the cluster size due to varying duplicate counts; (2) The errors during the sequencing stage such as PCR errors, pre-sequencing procedure, sampling errors that occur in Nanopore sequencing machine and errors of the translation between signal to read by the basecaller; and (3) the heart of the challenges of clustering DNA strands for DNA storage is the fact that the computation of a distance matrix ($\mathcal{O}(n^2)$ where $n$ is the number of reads) based on the edit distance between each pair ( $\mathcal{O}(\ell^2)$ where $\ell$ represents the length of the reads~\citep{landau1989fast}) of reads is not scalable for typical DNA storage datasets that are very big.



\hadas{Somthing about that the errors causes throw away "good" strands because of the errors in them}
%Our objective 
Our work addresses the concerns of both Nanopore sequencing and clustering DNA storage by proposing a novel approach: searching for similarity directly in the raw analog DNA signals rather than the discrete DNA reads. By exploiting the raw Nanopore signals which contain significantly more information compared to the discrete post-basecaller read. More specifically we proposed a deep neural network that aims to learn an effective representation of DNA signals such that the similarity measure between them will be much faster and more accurate than edit distance on the DNA strands. Moreover, this approach leads to a paradigm shift in DNA data storage since it eliminates the bascalling stage (see Figure~\ref{}) and significantly reduces both time and the errors introduced during the translation between signals and reads.
We perform extensive experiments on special datasets to highlight the effectiveness of our designed solution and the superior performance over state-of-the-art DNA strand edit distance.


In summary, the key contributions of our work are as follows: 
\begin{itemize}
    \item We are the first to exploit the potential of the raw DNA signal for the retrieval stage of DNA  storage.   
    \item The proposed approach significantly reduces sample exclusion because it uses the continuous dimension of electrical signals, which reduces the loss of information during the translation to the discrete dimension after basecalling.
    \item The proposed approach demonstrates the ability to achieve between 1 to 3 order-of-magnitude faster computation times while producing clusters with high enough quality to allow data reconstruction.
\end{itemize}

The rest of this paper is organized as follows: 

\begin{figure}[ht]
        \centering
        \includegraphics[width=1\linewidth]{figs/model_comparison.pdf}
        \caption{ENTER.}
        \label{fig:model}
\end{figure}
% Section~\ref{problemstate} defines the problem, and Section~\ref{relatedwork} reviews related work. Section ~\ref{datasets} introduces the uniqueness of the datasets and their creation, Section~\ref{solution} describes the proposed deep learning model, and Section~\ref{results} presents an evaluation of the trained ML models across different experiments. Section~\ref{application} uses the trained ML models for applications in the DNA storage pipeline, and Section~\ref{conclusion} concludes the paper.





%  By embedding the raw signals directly in an architecture composed of convolutional neural network (CNN) layers, long-short-term memory layers (LSTM), and linear layers, we bypass the limitations associated with clustering based on the A/T/C/G alphabet, allowing us to cluster raw signals before passing them through the basecaller. 

==> newsections/methodology.tex <==
\subsection{Datasets Construction}\label{sec:datacreate}

Public DNA storage datasets do not share the raw signals, Therefore, it is necessary to create our datasets from real experiments that map raw signals to their corresponding DNA reads. 

Each experiment in the DNA storage requires the 4 stages present in Section~\ref{intro}. First, choose an error-correcting code and generate a design file as part of the \textit{``encoding''} stage. Then \textit{``synthesis''} stage performed with \say{Twist Bioscience}, followed by a \textit{``sequencing''} stage, the DNA sequencer process lasts approximately $72$ hours. Then basecalling is performed on the DNA reads, which takes approximately a week. Lastly, creating the our signal-strand dataset lasts between $6-30$ days. 

Table~\ref{fig:exptable} shows three design files and their corresponding Nanopore sequencing experiments \footnote{The \say{Microsoft Experiment} design file is taken from~\citep{srinivasavaradhan2021trellis} and the sequenced data is from~\citep{sabary2024reconstruction}. The \say{Deep DNA Test} and \say{Deep DNA Pilot} design file and sequenced data are from ~\citep{bar2021deep}.}. The table outlines three different experiments that vary the number of clusters, the length of the DNA strands, and the average edit distance between strands in the design files, therefore resulting in high variability in key parameters for the proposed datasets.

Our datasets were obtained by brute-force calculating the edit distance between each DNA read produced by the basecaller and the original strands from the respective design file.
\hadas{maybe add for more information about the experiments appendix}



\begin{table}[t]
\centering
\caption{Experiments differences}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Experiment} & \textbf{No. Clusters} & \textbf{Strand Length} & \textbf{Avg Edit Dist.} & \textbf{Avg No. Copies} & \textbf{Avg Strand Length post Basecalling} & \textbf{Time Length Creation} \\
\hline
Microsoft Experiment & $10,000$ & $110$ & $52.6376$ & $300$ & $211$ & $18$ days \\
\hline
Deep DNA Pilot & $1,000$ & $140$ & $64.4932$ & $1,300$ & $240$ & $6$ days \\
\hline
Deep DNA Test & $110,000$ & $140$ & $4.0328$ & 10 & $243$ & $30$ days \\
\hline
\end{tabular}
}
\label{fig:exptable}
\end{table}

\subsection{Architecture}
We propose a deep-learning-based algorithm for computing similarity between the raw DNA signals. This is done by leveraging the Dorado basecaller~\citep{dorado2024} which is an open-source basecaller for Oxford Nanopore reads and the state-of-art among basecallers. Our technique is to use selected layers with their pre-trained weights from Dorado coupled with the ArcFace loss which will be discussed in Section~\ref{}. This way our model learns a representation of the DNA signals.


The input to the model are the raw DNA signals which are of length $3000$\footnote{the standard signal length in DNA storage datasets typically reaches up to $3000$ units, for $95\%$ of the cases, we uniformly reshaped all of the signals to this length using common techniques}. Initially, convolutional layers are deployed to extract salient features from the raw input signals through a sequence of convolutional operations, capturing critical patterns essential for the basecalling task. Following are recurrent layers (LSTM) that capture the sequential nature of the DNA sequence. They process the outputs from the convolutional layers, considering the order and dependencies between the nucleotides. The data is then passed through linear layers, which perform a linear transformation to align the processed features with the final output space. This is followed by a Clamp layer that ensures that the scores used for predicting the DNA sequence are within a specified range.


Thus, we utilize those pre-trained layers of Dorado, truncating its architecture after those layers, which outputs a size of $1024$. Subsequently, we append a linear layer with dimensions $1024 \times 500$, where $500$ represents the number of classes. 


\subsection{The Loss Function}

Considering all the errors in the sequencing model as presented in Section~\ref{intro} and the big datasets of DNA storage with a large number of clusters the solution needs to distinguish between the different signals in a way that there will not be overlap between the different clusters meaning in the embedding space the signals from the same cluster have to be close but far from signals from other clusters. Arcface or Additive Angular Margin Loss~\citep{deng2019arcface} is a loss function used in the state-of-the-art face recognition task. It is capable of handling tens of billions of classes (individual faces). Unlike Euclidean Distance, ArcFace loss calculation uses Geodesic Distance on a hypersphere which is a higher dimension space compared to Euclidean Distance. It is designed to enhance the discriminative power of the feature embeddings produced by a NN. ArcFace loss achieves this by enforcing a margin between the features of different classes in the angular space, making the decision boundary more distinct. Specifically, it adds an angular margin penalty to the target angles in the softmax function, which forces the NN to learn more separable features ~\citep{khan2024improvised}. The loss uses a cosine similarity in its implementation.
Given $\mathbf{A}, \mathbf{B}$ vectors of length $n$:
\begin{align*}
    \text{Cosine Similarity} = \cos(\theta) = \frac{\mathbf{A} \cdot \mathbf{B}}{\|\mathbf{A}\| \|\mathbf{B}\|} = \frac{\sum_{i=1}^{n} A_i B_i}{\sqrt{\sum_{i=1}^{n} A_i^2} \sqrt{\sum_{i=1}^{n} B_i^2}}
\end{align*}

This results in a more compact clustering of features from the same class and a wider separation between features of different classes. This loss function assists deeply in quantifying the similarity between the different signals see Figure~\ref{fig:softarch} for the differences between the common softmax loss and the ArchFace loss.

\begin{figure}[ht]
        \centering
        \includegraphics[width=1\linewidth]{figs/softmaxarchface.png}
        \caption{The image illustrates how ArcFace pushes feature vectors of different classes away from the decision boundary, with the angular margin ensuring distinct boundaries between identities.}
        \label{fig:softarch}
\end{figure}

Thus $\mathbf{x_i}\in \mathbb{R}^{d}$ denotes the deep feature of the $i$-th signal sample in a batch, belonging to the $y_i$-th class. $\mathbf{W}_j \in \mathbb{R}^{d}$ denotes the $j$-th column of the weight matrix of the fully connected layer $\mathbf{W}\in \mathbb{R}^{d\times n}$ where The embedding feature dimension $d$ and number of classes $n$  is set to 1024 and 500 correspondingly in this paper. $\mathbf{W}_j$ corresponding to class $j$

The output logit is obtained by taking the dot product of $\mathbf{W}^{T}_{j}\mathbf{x_i} = \|\mathbf{W}^{T}\|\|\mathbf{x}\|\cos{\theta_j}$, where $\theta_j$ denotes the angle between the weight vector $\mathbf{W}_j$ and feature vector $\mathbf{x_i}$. First the embedding feature $\mathbf{x_i}$ is fixed  $\|\mathbf{x_i}\|_2$ by $l_2$ normalization
and re-scale it to $s$ thus the embedding
features are distributed on a hypersphere with a radius
of $s$. Second  $\mathbf{W}_j$ is normalize by $l_2$ to 1 $\|\mathbf{W}_j\|_2=1$. Moreover, an additive angular margin penalty $m$ is added between $\mathbf{x_i}$ and $\mathbf{W}_{y_i}$
to simultaneously enhance the intra-class compactness and inter-class discrepancy. Mathematically, this can be expressed as:
\begin{align*}
    L = -\frac{1}{N}\sum_{i=1}^{N}\log{\frac{e^{s\cos{\theta_{y_i+m}}}}{e^{\cos{\theta_{y_i+m}}} + \sum_{j=1,j\neq y_i}^{n}e^{s\cos{\theta_j}}}}
\end{align*}



==> newsections/new_ev_hadas.tex <==
We examine two aspects of the proposed signal-based approach. First, we analyze our signal embeddings through comparisons with both edit distance-based methods and existing DNA embedding models. Second, we assess the clustering performance of our approach through comprehensive representation and accuracy analyses. We conduct our evaluations on three diverse datasets: \emph{Microsoft Experiment}, \emph{Deep DNA Pilot}, and \emph{Deep DNA Test}.  The results demonstrate both the accuracy and computational advantages of our method compared to existing approaches.

\begin{table}[t!]
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset} & \textbf{Size} & \textbf{Cluster Size} & \textbf{Use Case} \\
\midrule
Microsoft Exp. & 16,109 & Medium  & Practical deployment \\
Deep DNA Test & 739 & Small  & Baseline performance \\
Deep DNA Pilot & 63,849 & Large  & Large-scale validation \\
\bottomrule
\end{tabular}
}
\caption{Overview of the three datasets created from the experiments.}
\label{TABLE_DATASETS}
\end{table}
From each dataset, we selected subsets containing $50$ clusters to ensure a balanced comparison while maintaining computational feasibility. As shown in Table~\ref{TABLE_DATASETS}, \emph{Deep DNA Pilot} ($63,849$ samples, large clusters) is our large-scale validation dataset and presents challenging conditions for data retrieval due to the huge cluster sizes. In contrast, \emph{Deep DNA Test} ($739$ samples, small clusters) provides a controlled baseline for evaluating performance presents challenges to learn embeddings that distinguish between clusters. Finally, \emph{Microsoft Experiment} ($16,109$ samples, medium clusters) strikes a balance in scale and practical deployment considerations. These distinct characteristics ensure a comprehensive assessment of DNA storage clustering methods.

Each dataset provides both DNA signals and their corresponding sequenced reads, enabling direct comparison. To evaluate, we constructed binary similarity matrices for each dataset, where matrix entry $[i,j]$ equals $1$ if signals $i$ and $j$ belong to the same cluster, and $0$ otherwise. This ground truth serves as the baseline for our quantitative analysis and allows for systematic evaluation of clustering accuracy.
\subsection{Performance Analysis of Signal Embeddings}
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/mic_exp_roc_curve.pdf}
        \caption{\say{Microsoft Experiment}}
        \label{fig:microck}
    \end{subfigure}
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/omer_exp_roc_curve.pdf}
        \caption{\say{Deep DNA Pilot}}
        \label{fig:omerrock}
    \end{subfigure}
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/other_exp_roc_curve.pdf}
        \caption{\say{Deep DNA Test}}
        \label{fig:otherrock}
    \end{subfigure}
    \caption{Comparison of DNA signal similarity with \textit{signal-model} embeddings and DNA sequence similarity with edit-distance across datasets.}
    \label{fig:all_experiments}
\end{figure*}
\subsubsection{Comparison with edit distance}
We evaluate the performance of the \textit{signal-model}'s embedding-based similarity approach against traditional edit-distance methods applied to DNA reads for clustering. The evaluation focuses on both accuracy and computational efficiency.

To assess accuracy, we generated five distance matrices for each dataset: one cosine similarity matrix for the \textit{signal-model} (based on ArcFace loss~\cite{deng2019arcface}) and four edit-distance matrices with varying depth constraints. The depth constraint $k$ determines the range of possible edit-distance values $\{0, 1, \ldots, k\}$, where $k$ bounds the number of allowed insertions, deletions, or substitutions. We selected $k$ values of $10$, $20$, $50$, and $200$, approximately corresponding to $5\%$, $10\%$, $25\%$, and $100\%$ of our experimental DNA storage reads length (see~Table \ref{tab:exptable}). 

\begin{figure}[!t]
    \centering
        \includegraphics[width=0.8\columnwidth]{figforpaper/timing-dna111.pdf}
        \caption{Computation times across three datasets. For the \textit{signal-model}, this includes embedding generation and cosine similarity calculations, while for strand-\(k=xx\) models it covers edit-distance computations. Red crosses mark entries where the runtime exceeded 30 hour.}
        \label{fig:computation-time}
\end{figure}

An important distinction between the methods lies in their similarity measures. While edit-distance provides discrete thresholds corresponding to specific numbers of edits, the \textit{signal-model}'s cosine similarity offers continuous values ranging from $-1$ to $1$, where $1$ indicates perfect similarity.

Using these matrices, receiver operating characteristic (ROC) plots were generated. The ROC curve illustrates the trade-off between the true positive (TP) and false positive (FP) values of an ML model. Figure~\ref{fig:all_experiments} presents ROC curves comparing the \textit{signal-model} against the four baseline models with varying depth ($k$) values. Models with better performance exhibit ROC curves closer to the top-left corner, indicating a higher TP rate and a lower FP rate. A random model aligns with the diagonal identity line, while the area under the ROC curve (AUC) quantifies performance, normalized to $[0,1]$, where $1$ represents perfect classification.

The results demonstrate that the \textit{signal-model} achieves higher accuracy than the strand-based models across all experiments. For the \say{Microsoft Experiment}, the \textit{signal-model} attains an AUC of $0.99$, significantly outperforming the strand-$k=200$ ($0.81$), strand-$k=50$ ($0.80$), strand-$k=20$ ($0.57$), and strand-$k=10$ ($0.51$) models. The sharp turn and linear increase in all curves reflect read pairs exceeding the $k$-threshold, rendering them equally distant. The strand-$k=200$ model is the closest in performance to the \textit{signal-model}, as it effectively approximates an unbounded edit-distance calculation over the read length. However, this comes with significantly higher computational complexity.

Similar trends appear for the \emph{Deep DNA Pilot} and \emph{Deep DNA Test} datasets (Figures~\ref{fig:all_experiments}(\subref{fig:omerrock}) and~\ref{fig:all_experiments}(\subref{fig:otherrock})). Notably, the \emph{Microsoft Experiment} achieves better performance because the evaluation clusters share the same data distribution as the training set, although the specific clusters used for evaluation were unseen during training.

Regarding computational efficiency, Figure~\ref{fig:computation-time} illustrates the time required for similarity matrix computation across all experiments. The \textit{signal-model} demonstrates remarkable efficiency, requiring \textbf{1 to 3 orders of magnitude less time} compared to strand-based approaches. For the strand-$k=xx$ models, computation times increase linearly with $k$, while the \textit{signal-model} maintains consistent performance regardless of sequence complexity.

\subsubsection{Comparison with DNA embedding models}
% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[b]{0.30\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/mic_exp_roc_curve_LM.pdf}
%         \caption{\emph{Microsoft Experiment}}
%         \label{fig:microckLM}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.30\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/other_exp_roc_curve_LM.pdf}
%         \caption{\emph{Deep DNA Test}}
%         \label{fig:otherrockLM}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.30\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/omer_exp_roc_curve_LM.pdf}
%         \caption{\emph{Deep DNA Pilot}}
%         \label{fig:omerrockLM}
%     \end{subfigure}
%     \caption{DNA signal similarity compared to DNA sequence embedding across the datasets}
%     \label{fig:all_experiments_rocLM}
% \end{figure*}
To further validate the \textit{signal-model}'s approach, we compare against open sourced state-of-the-art DNA sequence embedding models: \textit{gena-lm-bert-base} (GLBB), \textit{gena-lm-bert-large-t2t} (GLBL)~\cite{fishman2023gena}, and \textit{DNABERT}~\cite{ji2021dnabert}. The GENA-LM models comprise a family of foundational models specifically designed for long DNA sequences, employing transformer-based architectures pre-trained on extensive human DNA sequence data. While the base version (GLBB) uses a standard BERT architecture, the large version (GLBL) incorporates additional transformer layers and attention mechanisms optimized for DNA sequences. DNABERT offers a specialized BERT model adapted for DNA sequences, incorporating $k$-mer embedding strategies to capture local sequence patterns. It employs a bidirectional encoder architecture specifically tuned for genomic data, with pre-training objectives designed to capture biological sequence properties.

In terms of embedding dimensionality, \textit{DNABERT} and \textit{gena-lm-bert-base} produce $768$-dimensional vectors, while \textit{gena-lm-bert-large-t2t} generates $1024$-dimensional embeddings matching our \textit{signal-model}'s dimensionality. While these models excel at capturing biologically relevant features in natural DNA sequences, they may not be optimally suited for synthetic DNA storage applications where the sequences don't necessarily follow natural biological patterns. 

ROC curves were created to compare these approaches. Table~\ref{DNA--TABLE} provides a unified comparison of both metrics, accuracy (AUC) and computational efficiency (Time), across four models on the three datasets. Our \textit{signal-model} approach significantly outperforms existing DNA models, achieving superior AUC scores ($0.92$--$0.99$) compared to ($0.6$--$0.7$) for the other DNA-based models. In terms of computational efficiency, our \textit{signal-model} processes the \emph{Microsoft Exp} dataset in $11.57$ seconds compared to $99$--$173$ seconds for other models, demonstrating up to 15x speedup while maintaining higher accuracy.
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Metric} & \textbf{GLBB} & \textbf{GLBL} & \textbf{DNABERT} & \textbf{\textit{signal-model}} \\
\midrule
\textbf{Microsoft Exp} & AUC & 0.64 & 0.70 & 0.60 & 0.99 \\
& Time[s] & 103.84 & 173.52 & 99.25 & 11.57 \\
\midrule
\textbf{Deep DNA Test} & AUC & 0.64 & 0.70 & 0.57 & 0.92 \\
& Time[s] & 1.56 & 3.53 & 3.00 & 1.49 \\
\midrule
\textbf{Deep DNA Pilot} & AUC & 0.60 & 0.70 & 0.56 & 0.94 \\
& Time[s] & 156.14 & 371.91 & 274.93 & 98.07 \\
\bottomrule
\end{tabular}}
\caption{Performance comparison of \textit{signal-model} and DNA embedding models across datasets.}
\label{DNA--TABLE}
\end{table}

\subsubsection{Comparison with DTW}
We also evaluated the similarity of our DNA signal model against Dynamic Time Warping (DTW). Specifically, we utilized the standard implementation of DTW as described in~\cite{senin2008dynamic} and FastDTW~\cite{salvador2007toward}, an approximate algorithm designed to achieve optimal or near-optimal alignments with linear time and memory complexity.
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Algorithm} & \textbf{AUC} & \textbf{Time} \\
\midrule
\textbf{\textit{signal-model}} & 0.92 & 1.49[sec] \\
\midrule
\textbf{DTW} & 0.44 & 20.97[days] \\
\midrule
\textbf{FastDTW} & 0.47 \\
\bottomrule
\end{tabular}}
\caption{Performance comparison of \textit{signal-model} to DTW variations on the {\emph{Deep DNA Test}} dataset.}
\label{DTWTABLE}
\end{table}
ROC curves were generated for the \textit{signal-model}, DTW, and FastDTW using the {\emph{Deep DNA Test}} dataset. Table~\ref{DTWTABLE} presents a comparison of the AUC for accuracy and the corresponding computation times. The results demonstrate that the \textit{signal-model} significantly outperforms both DTW and FastDTW in accuracy (by over $40\%$) and computational efficiency, achieving results in seconds compared to the days required by DTW approach.

\subsection{Clustering Performance Analysis}
To evaluate the \textit{signal-model}'s clustering capabilities, we conduct a systematic analysis across two key dimensions: representation quality and accuracy metrics. Our evaluation employs hierarchical clustering~\cite{murtagh2012algorithms} with cosine similarity on the three datasets, comparing against widely adopted DNA data storage clustering algorithms: Clover~\cite{qu2022clover} and Microsoft's alg~\cite{rashtchian2017clustering} (which we independently implemented following their paper's description), using their suggested parameters. Beyond demonstrating better clustering performance, our \textit{signal-model} approach eliminates the need for the time-consuming basecalling phase (saving days of computation), while achieving better results compared to DNA-based clustering algorithms. This shows that classical clustering techniques, when applied to our signal-based embeddings, can effectively outperform DNA storage clustering methods.

\subsubsection{Representation Learning}
Figure~\ref{fig:tsneall} provides t-SNE visualizations across the three datasets, offering insights into cluster separability. The \emph{Microsoft Experiment} (Figure~\ref{fig:tsneall}(a)) exhibits well-defined cluster boundaries with clear separation in the embedding space, demonstrating the model's ability to effectively distinguish between different clusters under typical conditions. The \emph{Deep DNA Test} results (Figure~\ref{fig:tsneall}(b)), despite its sparse data distribution, the visualization demonstrates clear cluster separation, with distinct groupings spread across the embedding space.Additionally, the \emph{Deep DNA Pilot} (Figure~\ref{fig:tsneall}(c)) shows denser cluster formations, reflecting the increased complexity and challenging conditions inherent in larger-scale data. These visualizations across different experimental conditions demonstrate the robustness of our \textit{signal-model}'s approach in capturing meaningful features within DNA signal data.
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.43\columnwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-mic50.pdf}
        \caption{\emph{Microsoft Experiment}}
        \label{fig:Tsnemic}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.43\columnwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-other50.pdf}
        \caption{\emph{Deep DNA Test}}
        \label{fig:Tsneother}
    \end{subfigure}
    \vspace{2mm}
    \begin{subfigure}[b]{0.43\columnwidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{figforpaper/TSNE-omer50.pdf}
        \caption{\emph{Deep DNA Pilot}}
        \label{fig:Tsneomer}
    \end{subfigure}
    \caption{t-SNE analysis of the 50 clusters of each dataset.}
    \label{fig:tsneall}
\end{figure}

\subsubsection{Clustering Accuracy for DNA} For evaluating clustering performance in DNA storage applications, traditional clustering metrics are insufficient as they do not account for the unique characteristics of DNA storage. We adopt and extend the accuracy measure introduced by~\cite{rashtchian2017clustering}, specifically designed for DNA storage data retrieval tasks. Let $C$ represent the ground truth clustering and $\tilde{C}$ denote the predicted clustering output from an algorithm. We define the clustering accuracy $\mathcal{A}_{\gamma,\beta}$ with two key parameters: $\gamma$ controlling the minimum required overlap for correct cluster identification, and $\beta$ establishing the maximum allowed fraction of false positives. Formally: \begin{definition}[DNA Storage Clustering Accuracy]
For clusters $C$, $\tilde{C}$, with parameters $0.5 < \gamma \leq 1$\text{,} $0\leq \beta < 0.5$\text{,} and a minimum overlap threshold $N$, the accuracy of $\tilde{C}$ with respect to $C$ is:
\begin{equation}
{\fontsize{9pt}{11pt}\selectfont
\begin{aligned}
    \mathcal{A}_{\gamma,\beta}(C, \tilde{C}) = \max_{\pi} \frac{1}{|C|} \sum_{i=1}^{|C|} &\mathbf{1}\{\tilde{C}_{\pi(i)} \setminus |\tilde{C}_{\pi(i)} \cap C_i| \leq \beta|\tilde{C}_{\pi(i)}| \\
    &\text{and } |\tilde{C}_{\pi(i)} \cap C_i| \geq \min(N, \gamma|C_i|)\}
\end{aligned}}
\end{equation}
where $\pi$ is a mapping from $\{1,2,\ldots,|C|\}$ to $\{1,2,\ldots,\max(|C|,|\tilde{C}|)\}$.
\end{definition}

This definition extends the original formulation in~\cite{rashtchian2017clustering} in two significant ways. First, we introduce the parameter $\beta$ to allow for a controlled fraction of false positives, considering that DNA storage reconstruction algorithms are designed to handle and correct a certain level of errors~\cite{sabary2024reconstruction}. Second, we add the constant $N$ to accommodate varying cluster sizes, particularly important for large-scale cluster size. ~\cite{rashtchian2017clustering}'s accuracy is defined for $\beta=0$ and under the assumption that the output of sequencing is a small number of noisy DNA reads of each cluster reference.

The accuracy measure $\mathcal{A}_{\gamma,\beta}$ evaluates clustering quality through two essential conditions. The false positive condition $\tilde{C}_{\pi(i)} \setminus |\tilde{C}_{\pi(i)} \cap C_i| \leq \beta|\tilde{C}_{\pi(i)}|$ ensures that no more than a $\beta$-fraction of elements in each predicted cluster are incorrectly assigned. Additionally, the overlap condition $|\tilde{C}_{\pi(i)} \cap C_i| \geq \min(N, \gamma|C_i|)$ requires either a minimum absolute overlap of $N$ samples or a relative overlap of $\gamma$-fraction, whichever is smaller. This interpretation justifies the need for high accuracy and an error fraction: each underlying cluster represents one stored unit of information.
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/mic_clustering_results.pdf}
        \caption{\emph{Microsoft Experiment}}
        \label{fig:micclust}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/other_clustering_results.pdf}
        \caption{\emph{Deep DNA Test}}
        \label{fig:otherclust}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/omer_clustering_results.pdf}
        \caption{\emph{Deep DNA Pilot}}
        \label{fig:omerclust}
    \end{subfigure}
    \caption{Comparison to Microsoft algorithm. Figures (a) and (b) plot $\mathcal{A}_{\gamma,\beta}$ for varying $\gamma \in \{0.6, 0.7, 0.8, 0.9, 1.0\}$ and $N=200$. (c) plots $\mathcal{A}_{\gamma,\beta}$ for varying $N\in\{20,50,100,200,400\}$ due to \emph{Deep DNA Pilot} huge clusters that in this case $N=\min(N, \gamma|C_i|)$. All figures include plots for $\beta\in \{0,0.1,0.2\}$ as the false positive rate in the clusters. In (a) and (c) our Alg $\beta=0.1$, our Alg $\beta=0.2$ have the same accuracy.}
    \label{fig:clustering_results}
\end{figure*}

Figure~\ref{fig:clustering_results} presents accuracy comparisons between our hierarchical clustering algorithm, which leverages signal-model embeddings, and Microsoft’s state-of-the-art method for DNA data storage sequences~\cite{rashtchian2017clustering}. Clover was excluded from this comparison because it consistently underperformed. Each subplot captures the performance under distinct datasets and parameter variations, illustrating how accuracy changes in response to the false-positive rate $\beta\in\{0,0.1,0.2\}$, the overlap determined by the min between the $\gamma$ threshold, and the constant parameter $N$. In particular, $\beta$ governs how much noise is introduced into each cluster (higher $\beta$ indicates noisier clusters), while $\gamma \in \{0.6, 0.7, 0.8, 0.9, 1.0\}$ in Figures~\ref{fig:clustering_results}~(a) and~\ref{fig:clustering_results}(b), specifying how strictly a produced cluster must overlap with the original ground-truth cluster. In Figure~\ref{fig:clustering_results}~(c), for the large cluster size dataset, we show accuracy as a function of \(N\), since the overlap is effectively determined by \(\min\bigl(N, \,\gamma \lvert C_i\rvert\bigr)\).

In Figure~\ref{fig:clustering_results}(a), our algorithm consistently achieves higher accuracy than Microsoft’s across all examined noise levels. While both methods experience slight decreases in accuracy under more stringent overlap requirements (larger $\gamma$), our algorithm remains comparatively robust, for smaller $\beta$ values our algorithm achieve $94\%$, while retaining accuracy above $60\%-70\%$ for larger $\beta$, whereas Microsoft’s method frequently hovers below $30\%$. In Figure~\ref{fig:clustering_results}(b), which corresponds to a smaller dataset, both algorithms show reduced performance due to tighter constraints on $\beta$ and $\gamma$. Nonetheless, our method still outperforms Microsoft’s: for $\beta=0.2$, we achieve $50\%$ accuracy versus Microsoft’s $30\%$. For both plots, $N$ is set to $200$, as it is enough for reconstruction purposes and does not affect the overlap fraction.

Finally, Figure~\ref{fig:clustering_results}(c) presents the results for the large dataset, where the effect of \(\gamma\) diminishes because \(N\) is effectively bounded by \(\min(N,\gamma|C_i|)\). Our algorithm achieves perfect accuracy at moderate \(N\) values and remains resilient even as \(N\) increases to 400. By contrast, Microsoft’s approach yields a vast majority of clusters of size~1 and merges many sequences into a few large clusters, resulting in stable but substantially lower accuracy overall. In fact, it creates 90\% of its clusters with size~1 and 97\% with sizes below~19, which are redundant given the dataset’s average cluster size of $1,300$. Moreover, in the few large clusters it does form, it often merges distinct groups, adversely affecting the \(\beta\) fraction and explaining the 20\% accuracy boost observed at \(\beta=0.2\). Nevertheless, that boost is overshadowed by the balanced cluster-size distribution our method maintains, as evidenced by its perfect accuracy for \(\beta=0.1\). Overall, these findings confirm that our hierarchical signal-model algorithm outperforms the existing state-of-the-art across various noise levels, overlap thresholds, and dataset sizes, underscoring its suitability for a successful reconstruction of DNA data storage tasks. 
\subsubsection{Clustering Robustness}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Dataset} & \textbf{Alg} & \textbf{Recall} & \textbf{Precision} & \textbf{F1} & \textbf{No. Clusters} \\
\midrule
\multirow{3}{*}{\textbf{Microsoft exp}} & \textit{signal-model} & 0.794 & 0.994 & 0.883 & 145 \\
& clover & 0.13 & 0.042 & 0.064 & 40 \\
& Mic. & 0.688 & 0.171 & 0.274 & 26 \\
\midrule
\multirow{3}{*}{\textbf{Deep DNA Test}} & \textit{signal-model} & 0.650 & 0.563 & 0.604 & 45 \\
& clover & 0.212 & 0.024 & 0.044 & 33 \\
& Mic. & 0.56 & 0.598 & 0.578 & 75 \\
\midrule
\multirow{3}{*}{\textbf{Deep DNA Pilot}} & \textit{signal-model} & 0.357 & 0.953 & 0.519 & 387 \\
& clover & 0.39 & 0.101 & 0.161 & 44 \\
& Mic. & 0.577 & 0.668 & 0.619 & 2090 \\
\bottomrule
\end{tabular}}
\caption{Comparison of clustering algorithms across datasets.}
\label{tab:clustering_comparison}
\end{table}
Table~\ref{tab:clustering_comparison} presents an evaluation of our algorithm against standard clustering metrics across all datasets. The performance is measured using three key metrics: Recall ($\frac{TP}{TP + FN}$), which indicates the model's ability to identify all positive samples; Precision ($\frac{TP}{TP + FP}$), which measures the model's accuracy in positive predictions; and F1 score, the harmonic mean of precision and recall that provides a balanced assessment of the model's overall performance.

The results demonstrate consistent strong performance across different experimental conditions. On the \emph{Microsoft Experiment} dataset, our algorithm achieves superior performance across all metrics. For the \emph{Deep DNA Test} dataset, while our and Microsoft algorithms show comparable performance, our approach maintains an edge in both Recall and F1 scores. Even on the challenging \emph{Deep DNA Pilot} dataset, which features exceptionally large clusters, our algorithm achieves a competitive F1 score of $0.519$ compared to Microsoft's $0.619$. Notably, while our and Microsoft algorithms process the complete dataset, Clover's approach discards a significant portion of the input reads—retaining only $3\%$ ($486$ of $16,109$) reads in the \emph{Microsoft Experiment} and less than $1\%$ ($476$ of $63,849$) in the \emph{Deep DNA Pilot}. We achieve similar results with Microsoft alg for Rand-Index ($0.98$), Homogeneity($\pm 0.8$), Completeness ($\pm 0.8$) and V-measure($\pm 0.8$) scores, while Clover does not.


==> newsections/related____work.tex <==
%the edit distance computetion
Direct utilization of the raw signal is challenging since, to the best of our knowledge, no previous work in DNA storage has directly exploited the DNA signals for processes such as clustering, reconstruction, and error correction in the retrieval stage. DNA clustering algorithms often suffer from high computational time and compromised accuracy. However, they try To address the edit-distance quadric computation complexity achieved by dynamic programming methods~\citep{landau1989fast,gusfield1997algorithms} by proposing several methods. First, restrict the computation depth of the edit-distance to mitigate the complexity as demonstrated in~\citep{bao2011seed}. Second, the edit-distance can be calculated based on fixed-sized short sub-strings, as implemented in Starcode~\citep{zorita2015starcode} using short DNA bar-codes.\hadas{Maybe eliminate} Another approach leverages heuristic similarity instead of edit-distance to expedite processing times, as demonstrated in Clover~\citep{qu2022clover} utilizing a tree structure.
%and (2) \textit{filtering} techniques to reduce the number of pairwise comparisons.


%DTW SIGNAL DOMAIN
In the signal domain, a common method for comparing signals is Dynamic Time Warping (DTW)~\citep{senin2008dynamic}. DTW is a technique designed to compare two time series sequences with varying lengths whose data points are not aligned, much like strands in the discrete domain, allowing for insertions, deletions, and substitutions. Similar to edit-distance, DTW's computational complexity is quadric. Given that signal lengths are typically ten times longer than DNA strands, DTW computation becomes impractical for large datasets that are used in DNA storage applications. Similar to the edit distance while the base case of DTW has a quadric complexity, various optimizations, such as limiting the diagonals, applying lower bounds, or utilizing hardware acceleration, can speed up the process~\citep{rakthanmanon2012searching}
However, in our specific case, where we are dealing with many-to-many comparisons for DNA data storage applications the performance is not sufficient.



%DNA EMBEDDINGS MODEL
We acknowledge prior works, such as ~\citep{ji2021dnabert, li2021bioseq}, focused on embedding-based DNA sequence representation. Unlike our approach, these models are designed to capture biological structures, such as proteins or genes, and are typically task-specific. In contrast, DNA data storage requires a universal solution for encoding synthetic data, where the goal is to reconstruct the original data without aligning it to biological structures learned by their models.




 
 
% Several DNA clustering algorithms in bioinformatics and metagenomics, such as UCLUST~\citep{leproust2010synthesis}, CD-HIT~\citep{fu2012cd}, and USEARCH ~\citep{srinivasavaradhan2021trellis}, use different methods to deal with the two challenges. One approach involves using greedy methods for filtering, such as identifying common short sub-sequences as a preliminary step before edit-distance computation. Location Sensitive Hashing (LSH), which is used in~\citep{antkowiak2020low, rashtchian2017clustering, ben2023gradhc}, is another emerging method that limits the edit-distance calculation to strands that share the same LSH value to make filtering more efficient. 


 
 





% Given the focus on signal domain analysis in this study, it is crucial to initially address an approximate solution (2).


% Meshclust \cite{james2018meshclust} reduces the parameter sensitivity problem by using the mean-shift algorithm. 

% Filtering - 
% greedy algorithms

% DNA-clustering algorithms from bioinformatics and metagenomics:
% UCLUST [14]
% CD-HIT \cite{fu2012cd} - a greedy incremental algorithm; no guarantee optimal % solution.
% UCLUST [25], based on USEARCH [25], finding common short words between sequences % [26].
% DNACLUST [16] 
% SEED \cite{bao2011seed} - hashing techniques and interval seeding. 

% LSH
% \cite{antkowiak2020low} developed a location-sensitive, hash-based. 
% Microsoft algorithm,
% \cite{rashtchian2017clustering} uses a minimal hash algorithm
% Grad-HC


% Approximation - 

% partially computation length
% using k 
% Starcode \cite{zorita2015starcode} using edit matrices. 
% Clover \cite{qu2022clover} - avoiding computation of the Levenshtein distance, using a tree structure.
% 

%old
%In the DNA strands clustering phase, a substantial number of clusters (ranging from 1,000 to 100,000) typically contain varying numbers of samples (ranging from 10 to 1,000) each. DNA strands clustering involves computing the similarity between pairs of strands using edit-distance, which presents two main challenges: (1) the computational complexity of pairwise comparisons being $\mathcal{O}(n^2)$ where $n$ is the number of strands, and (2) the $\mathcal{O}(\ell^2)$ complexity of edit-distance computation, where $\ell$ is the length of the strands. Therefore, DNA clustering algorithms address these challenges by employing (1) \textit{Filtering} techniques to reduce the number of pairwise comparisons and (2) \textit{approximation} methods to expedite edit-distance calculations. Both approaches aim to decrease time complexity with minimal loss of accuracy.$

==> sections/motivation.tex <==




\textbf{Challenges in Clustering DNA Strands:} In the realm of DNA data storage retrieval, a pivotal stage in the pipeline involves clustering billions of strings based on their edit-distance, which quantifies the minimum number of edits—insertions, deletions, or substitutions—needed to transform one string into another \cite{ristad1998learning}. The datasets within this domain typically comprise a vast number of small clusters that exhibit significant separation in the edit-distance metric space. However, existing clustering algorithms often falter in this scenario due to their inability to cope with either prolonged computational time or compromised accuracy. While approximation algorithms and tools like metric embeddings and locality-sensitive hashing (LSH) offer promising avenues by sacrificing some accuracy for substantial reductions in runtime, their applicability to edit-distance remains inadequately understood. 

At the heart of the challenges in clustering DNA strands for storage lies the impracticality of computing a distance matrix between every pair of input strands due to the sheer volume of data. Moreover, the quadratic time complexity of edit-distance algorithms in relation to the length of the strands exacerbates this issue. Our work addresses the latter concern by proposing an innovative approach: embedding DNA signals while preserving similarity. 

\textbf{Novelty of Proposed Approach:} Our paper introduces a paradigm shift in the field of DNA data storage retrieval by leveraging deep neural network embedding on Nanopore signals instead of the traditional ACGT alphabet of DNA strands. This novel approach diverges from conventional methods by focusing on the direct analysis of Nanopore signals, which offers several advantages. By embedding the signals directly, we bypass the limitations associated with clustering based on the ACGT alphabet, allowing us to cluster the data before subjecting it to the Nanopore procedure. This preemptive clustering step significantly reduces errors introduced during sequencing, leading to more accurate reconstruction of the original sequences.

Furthermore, our approach opens up avenues for the development of alternative basecalling techniques. Rather than relying on the current Nanopore model, which operates on individual signals, our method enables the development of basecallers that can analyze the entire cluster of signals collectively. This holistic approach enhances the accuracy and reliability of basecalling, as it leverages the collective information from multiple signals to infer the original ACGT sequence with greater precision.

Overall, the novelty of our proposed approach lies in its ability to streamline the DNA data storage retrieval process, mitigate errors introduced during sequencing, and pave the way for the development of more efficient basecalling techniques. By embracing this paradigm shift, we aim to revolutionize the way DNA data storage systems are accessed and utilized, ultimately advancing the field towards more reliable and scalable storage solutions.


